Unitarity Bound on Extended Higgs Sector with Higher Dimensional Operator

We study the perturbative unitarity bound given by higher dimensional bosonic operators up to dim-6 for the two-Higgs-doublet model (2HDM). They lead to new physics beyond the Standard Model. We point out that such operators can lead to a larger cross-section in the vector boson fusion channels for the scalars, compared to the tree-level 2HDM. We have obtained limits on a few bosonic operators up to dim-6 for 2HDM, by ensuring unitarity of the S-matrix.

==> Chapter6/chapter6.tex <==
%\chapter*{Chapter 6 :}
%\chapter*{Chapter 6 : Meta-stability in Extended Standard Model }
\chapter{Metastability in Extended Scalar Sectors of the Standard Model}
\label{chap:MetaSMextended}
\linespread{0.1}
\graphicspath{{Chapter6/}}
\pagestyle{headings}
%{\bf{\Huge Chapter 6 }}\\
%\noindent\rule{5.5cm}{1.5pt} \\
%\vspace*{0.8cm}\\
%{\bf{\Huge Metastability in Extended Standard Model}}\\
\noindent\rule{15cm}{1.5pt} 
%\noindent\rule{14cm}{2.8pt} 
\section{Introduction}
 
It has been seen in the previous chapter that life time of the Universe is finite in the SM. It is important to explore if the new extra scalar field(s) of an extended scalar sector has an answer to this puzzle in its reserve.
In this work a $SU(2)_L$ singlet~\cite{Khan:2015ipa} or a doublet~\cite{Khan:2014kba} or a hyperchargeless triplet~\cite{NajimTrip} scalar is added to the SM and a $Z_2$-symmetry is imposed on these new models such that the $odd$ number of new scalar fields do not couple with the SM particles.
As the lightest neutral particle of the additional scalar sector cannot decay, it becomes stable and serves as a viable dark matter candidate which may saturate the relic abundance of the dark matter in the Universe.
As these new models contain various kinds of new scalar fields, the structure of scalar potential and the absolute stability bounds of the EW vacuum of the scalar potential which had been shown in Chapter~\ref{chap:EWSBextended} are rather complicated than that in the SM due to the involvement of more parameters. 


In this work, a detailed study of the metastability of the EW vacuum of Higgs potential in the extended scalar sector will be presented. Various kinds of phase diagrams will be drawn to illustrate the region of absolute stability, metastability, instability and the non-perturbativity on different parameter spaces of these extended scalar sectors. In the Section~\ref{SingletSMext}, the stability of the EW vacuum in the presence of a real singlet scalar will be discussed. In Sections~\ref{doubletexten} and~\ref{sec:ITM}, similar studies for the inert doublet model (IDM) and inert triplet model (ITM) will be elaborated.
%%%%%%%%%%%%%%%%%%%%%
\section{Singlet scalar extension of SM}\label{SingletSMext}
%%%%%%%%%%%%%%%%%%%%%%
Recent cosmological and astrophysical evidences suggest presence of cold dark matter (DM). A simple choice is to add a gauge singlet real scalar $S$ to the SM~\cite{Burgess:2000yq}. An additional $Z_2$ symmetry ensures the stability of $S$. The scalar modifies the Higgs effective potential, and can ensure vacuum stability up to $\mpl$.
Such extensions of SM have been discussed in the literature~\cite{Haba:2013lga,Kadastik:2011aa, Gabrielli:2013hma,Gonderinger:2009jp,Clark:2009dc,Lerner:2009xg,Cheung:2012nb,Lebedev:2012zw, EliasMiro:2012ay,Antipin:2013bya, Khan:2012zw,Grzadkowski:2001vb, Branchina:2013jra, Lalak:2014qua, Branchina:2014usa,Eichhorn:2014qka} in the context of vacuum stability.

In the context of SM, detailed studies of metastability has shown in Chapter~\ref{chap:MetaSM}. 
Along the same line, in this section, the studies of the metastable vacuum has been extended to the SM+$S$ model~\cite{Khan:2014kba}.
%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Effective potential and RGE running}
\label{EffpotScalar}
%\section{SM with an extra singlet scalar}
In this model, an extra real scalar singlet field $S$, odd under $Z_2$ symmetry, is added to the SM, providing a suitable candidate for dark matter. The corresponding Lagrangian density is given by,
%%%%%%%%%%%%%%%%%
\begp
\allowdisplaybreaks \beq
{\cal L}_{S}= \frac{1}{2} (\partial_{\mu} S) (\partial^{\mu} S) -V_0^S\nn
\eeq
\eegp
%%%%%%%%%%%%%%%%%%%%
with,
%%%%%%%%%%%%%%%%%
\begp
\allowdisplaybreaks \beq
V_0^S= \frac{1}{2} \overline{m}_S^2 S^2 +\frac{\kappa}{2} |\Phi|^2 S^2 +
 \frac{\lambda_S}{4!} S^4 \, ,
 \label{Vscalar}
\eeq
\eegp
%%%%%%%%%%%%%%%%%%%%
where, 
%%%%%%%%%%%%%%%%%
\begp
\allowdisplaybreaks \beq
\Phi=\begin{pmatrix}
G^+ \\ (h+v+iG^0)/\sqrt{2}
\end{pmatrix} \nn \, .
\eeq
\eegp
%%%%%%%%%%%%%%%%%%%%
After spontaneous EW symmetry breaking, DM mass $M_S$ is expressed as $M_S^2=\overline{m}_S^2  +\kappa v^2/2$.

SM tree level Higgs potential
%%%%%%%%%%%%%%%%%
\begp
\allowdisplaybreaks \beq
V_0^{\rm SM}(\phi)=-\frac{1}{2} m^2 h^2 + \frac{1}{4} \lambda h^4\nn\\
\eeq
\eegp
%%%%%%%%%%%%%%%%%%%%
is augmented by the 
SM+$S$ one-loop Higgs potential in Landau gauge using $\MS$ scheme, which is written as
%%%%%%%%%%%%%%%%%
\begp
\allowdisplaybreaks \beq
V_1^{{\rm SM}+S}(h)= V_1^{\rm SM}(h) + V_1^{S}(h). \nn
\eeq
\eegp
%%%%%%%%%%%%%%%%%%%%
The expression of $V_1^{\rm SM}(h)$ is given\footnote{Here $h$ is used instead of $\phi$, representing the SM-like Higgs field.} in eqn.~\ref{V1loop} and the one loop contribution of the singlet scalar can be written as~\cite{Lerner:2009xg, Gonderinger:2012rd},
%%%%%%%%%%%%%%%%%%
\begp
\allowdisplaybreaks \bea
V_1^{S}(h)&=&\frac{1}{64 \pi^2} M_S^4(h) \left[ \ln\left(\frac{M_S^2(h)}{\mu^2(t)} \right)-\frac{3}{2} \right], \nn
\eea
\eegp
%%%%%%%%%%%%%%%%%%%%
where,
%%%%%%%%%%%%%%%%%%
\begp
\allowdisplaybreaks \bea
M_S^2(h) &=& \overline{m}_S^2(t)  +\kappa(t) h^2(t)/2\, .
\nn
\eea
\eegp
%%%%%%%%%%%%%%%%%%%%
SM contributions are taken at two-loop level~\cite{Ford:1992pn, Martin:2001vx, Degrassi:2012ry, Buttazzo:2013uya}, whereas the scalar contributions are considered at one-loop only. 

For $h\gg v$, the effective potential can be approximated as
%%%%%%%%%%%%%%%%%
\begp
\allowdisplaybreaks \beq
V_{\rm eff}^{{\rm SM}+S}(h) \simeq \lambda_{\rm eff}(h) \frac{h^4}{4}\, ,
\label{efflamS}\eeq
\eegp
%%%%%%%%%%%%%%%%%%%%
with
%%%%%%%%%%%%%%%%%
\begp
\allowdisplaybreaks \beq
\lambda_{\rm eff}(h) = \lambda_{\rm eff}^{\rm SM}(h) +\lambda_{\rm eff}^{S}(h)\, ,
\label{lameffscalar}
\eeq
\eegp
%%%%%%%%%%%%%%%%%%%%
where $\lambda_{\rm eff}^{\rm SM}(h)$ can be found in eqn.~\ref{eq:effqurtic} and,
%%%%%%%%%%%%%%%%%%
\begp
\allowdisplaybreaks \bea
 \lambda_{\rm eff}^{S}(h)&=&e^{4\Gamma(h)} \left[\frac{\kappa^2}{64 \pi^2}  \left(\ln\left(\frac{\kappa}{2}\right)-\frac{3}{2}\right ) \right]\, . \label{efflamscalar}
\eea
\eegp
%%%%%%%%%%%%%%%%%%%%
As quartic scalar interactions do not contribute to wave function renormalization at one-loop level, $S$ does not alter  $\gamma(\mu)$ of SM and anomalous dimension of $S$ is zero~\cite{Gonderinger:2009jp}.  
All running coupling constants are evaluated at $\mu=h$.

The beta functions for the new physics parameters $\kappa$ and $\lambda_S$ are given in eqn.~\ref{eq:betasinglet}. $\overline{m}_S$ also evolves with energy. But as the beta functions of other parameters do not involve $\overline{m}_S$, its beta function is not considered in this discussion.
Here, new physics effects are included in the RGEs at one-loop only.
%%%%%%%%%%%%%%%%%%%%%%
\subsection{Singlet Scalar as a dark matter candidate}
\label{darksingletScalar}
%%%%%%%%%%%%%%%%%%%%%%
As it has already been discussed that the new extended real singlet scalar is odd under $Z_2$ symmetry, i.e., under this symmetry, $S\rightarrow -S$, but Standard Model particles are invariant. Due to $Z_2$ symmetry $odd$ numbers of the scalar fields $S$ do not couple with the SM particles. The particle $S$ is stable and it can be considered as a viable dark matter candidate.
This model can provide dark matter with almost all possible mass ranges which allowed from the relic density constraints of WMAP~\cite{Bennett:2012zja} and Planck~\cite{Ade:2013zuv} data. 

After EW symmetry breaking one can write the potential (see eqn.~\ref{Vscalar}) explicitly as,
%%%%%%%%%%%%%%%%%
\begp
\allowdisplaybreaks \beq
V_0^S=\frac{1}{2}\left(\overline{m}_S^2+\frac{\kappa v^2}{2}\right) S^2 + \frac{k v}{2} h S^2+\frac{\kappa}{4} h^2 S^2+\frac{\lambda_S}{24} S^4.
\label{VscalarExpand}
\eeq
\eegp
%%%%%%%%%%%%%%%%%%%%
$S$ is the scalar singlet under the SM gauge symmetry so there are no 4-point coupling like, $SSXX$ ($X$ is the SM vector boson or a fermion). The scalar field can annihilate to SM particles only $via$ Higgs exchange. $S$ is called a Higgs portal dark matter.
LHC has put a stringent bounds on the Higgs invisible decay width~\cite{Belanger:2013xza}. The decay width of $h$ to pair of $S$ is given by,
%%%%%%%%%%%%%%%%%
\begp
\allowdisplaybreaks \beq
\Gamma\left(h\rightarrow SS\right)= \frac{ v^2}{32\pi M_h }\kappa^2 \left(1-\frac{4 M_{\rm DM}^2}{M_{h}^2}\right)^{1/2}\,.
\label{decaywidthS}
\eeq
\eegp
%%%%%%%%%%%%%%%%%%%%
Also the direct detection experiments, XENON\,100~\cite{Aprile:2011hi,Aprile:2012nq} and LUX~\cite{Akerib:2013tjd} puts a bound on the dark matter mass from the non-observation of dark matter-nucleon scattering. DM direct detection involve the $h$-mediated $t$-channel process, $SN\ra SN$. The scattering cross-section is given by,
%%%%%%%%%%%%%%%%%
\begp
\allowdisplaybreaks \beq
 \sigma_{S,N} = \frac{m_r^2}{4 \pi} f_N^2 m_N^2\left(\frac{\kappa}{M_{\rm DM} M_h^2}\right)^2 \label{directcsS}
\eeq
\eegp
%%%%%%%%%%%%%%%%%%%%
where $f_N\approx0.3$ is the form factor of the nucleus. $m_r$ represents the reduced mass of the nucleus and the scattered dark matter particle.

With the invisible Higgs decay width at LHC and non-observation of dark matter in the direct detection experiment at the LUX and including indirect Fermi-LAT bounds, it has been shown in Refs.~\cite{Duerr:2015mva,Duerr:2015aka} that the dark matter mass below 50 GeV and $70-110$ GeV are excluded.
In the table~\ref{tableS1}, few benchmark points have been shown for low dark matter mass less than the half of the Higgs mass.
{\tt FeynRules}~\cite{Alloul:2013bka} along with {\tt micrOMEGAs}~\cite{Belanger:2010gh, Belanger:2013oya} have been used to compute relic density of scalar DM in SM+$S$ model. 
The main dominant contributions to the relic density in these region is $SS\ra b \bar{b}$.
%%%%%%%%%%%%%%%%
%\renewcommand*{\arraystretch}{15}{
\setlength\tablinesep{1pt}
\setlength\tabcolsep{10pt}
\begin{table}[h!]
\begin{center}
    \begin{tabular}{ | c | c |  c | c | c | c |}
    \hline
     $M_{DM}$ (GeV) & $\kappa$ & Relic density &$\sigma_{SI}$ ${\rm ({cm}^2)}$& Br($h\rightarrow S S$) in $\%$\\
    \hline
     $55$ & 0.007 & 0.1242 & $1.3\times10^{-46}$ & 1.83   \\
    \hline
     $56$ & 0.0045 & 0.1182 & $5.5\times10^{-47}$ & 0.72   \\
     \hline
     $58$ & 0.0018 & 0.1199 & $8.2\times10^{-48}$ & 0.121   \\
     \hline
     $60$ & 0.00075 & 0.1203 & $1.3\times10^{-48}$ & 0.013   \\
     \hline
             \end{tabular}
    \caption{\textit{ Benchmark points with dark matter mass $M_{DM}< M_h/2$, which is allowed from the relic density constraint on the DM of WMAP and Planck, $\Omega h^2=0.1198\pm 0.0026$ within 3$\sigma$ confidence level, direct detection LUX (2013) and Higgs invisible decay width from the LHC. }}
    \label{tableS1}
\end{center}
\end{table}
%%%%%%%%%%%%%%%%%%%%

In Fig.~\ref{fig:relicScalar}, how the relic density changes with the dark matter mass in this model, has been shown.
The plot generated for three different Higgs portal coupling $\kappa(M_Z)=0.05$ (black), $\kappa(M_Z)=0.10$ (brown), and $\kappa(M_Z)=0.15$ (red). 
Here the blue band corresponds to the relic density constraints from WMAP and Planck data allowed at 3$\sigma$ confidence level. The light red band region is excluded from the Higgs invisible decay width. 
For the $\kappa(M_Z)=0.05$, one can see that there are four regions in dark matter mass which cross the blue band, i.e., satisfy the relic density in the right ballpark.

The dark matter mass near the 50 GeV, the dominant part in the annihilation of relic density is $SS \ra b\bar{b}$ (79$\%$), $SS\ra W^{\pm}W^{\mp*}$\footnote{The virtual $W^{\pm*}$ can decay to quarks and leptons.} (8$\%$), $SS \ra c\bar{c}$(7$\%$), however these regions are not allowed from Higgs invisible decay width as well as from the direct detection data. For 70 GeV, the process $SS \ra b\bar{b}$ is about 52$\%$ and $SS\ra W^{\pm}W^{\mp*}$ is 40$\%$ of total annihilation cross-section.
Whereas for the dark matter mass around 160 GeV, the dominant contributions in the annihilation are, $SS \ra W^{\pm}W^{\mp}$ (48$\%$), $SS \ra hh$ (30$\%$) and in $SS \ra ZZ$ (22$\%$) are allowed from direct searches. Similarly for other values of $\kappa(M_Z)$, the relic density in the right ballpark can be found near the dark matter mass 400 GeV and 500 GeV. In this case dominant contributions are $SS \ra hh,t\bar{t}$.
%%%%%%%%%%%%%%%%%%
\begin{figure}[h!]
\begin{center}
{
\includegraphics[width=2.7in,height=2.7in, angle=0]{./Plots/ScalarRelivsMDM}}
\caption{ \textit{ Dark matter relic density $\Omega h^2$ as a function of the dark matter mass $M_{DM}(\equiv M_S)$ for different values of the portal coupling: $\kappa(M_Z)=0.05$ (black), $\kappa(M_Z)=0.10$ (brown), and $\kappa(M_Z)=0.15$ (red). The thin blue band corresponds to the relic density of the dark matter, $\Omega h^2=0.1198 \pm 0.0026$ (3$\sigma$) of the present the Universe.}}
\label{fig:relicScalar}
\end{center}
\end{figure}
%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%
\begin{figure}[h!]
\begin{center}
{
\includegraphics[width=2.7in,height=2.7in, angle=0]{./Plots/kappavsMDM}}
\caption{ \textit{ {\rm SM+}$S$ allowed parameter space in the $\kappa(M_Z)-M_{DM}$ plane in agreement with the relic density constraints, direct and indirect detection. Where the upper dotted, solid in the middle and the lower dotted blue line correspond to the relic density $\Omega h^2=0.112,0.1198$ and $0.1276$ respectively.}}
\label{fig:reliclmsvsmass}
\end{center}
\end{figure}

In Fig.~\ref{fig:reliclmsvsmass}, the relic density in $\kappa(M_Z)-M_{DM}$ plane for the high dark matter masses have been plotted.
In this plot the blue line (upper dotted) corresponds to the relic density $\Omega h^2=0.112$ (minimum relic density allowed from WMAP and Planck) and other two belong to $\Omega h^2=0.1198$ and $\Omega h^2=0.1276$ (maximum) respectively. The relic density band is almost like a straight line because for $M_{DM} > M_W, M_h$, the annihilation cross-section is proportional to $\frac{\kappa^2}{ M_{DM}^2}$.

%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%
\subsection{RGE running from $\mu=M_t$ to $\mpl$ in SM+$S$}
%%%%%%%%%%%%%%%%%%%%%%% 
The similar technique of the matching conditions of Section~\ref{MatchingSM} has been used to calculate all the coupling at $\mu=M_t$. After knowing the values of various coupling constants at $M_t$, full three-loop SM RGEs and one-loop RGEs for the scalar $S$ have been used to run them up to $\mpl$.

%%%%%%%%%
%\renewcommand*{\arraystretch}{15}{
\setlength\tablinesep{1pt}
\setlength\tabcolsep{5pt}
\begin{table}[h!]
\begin{center}
    \begin{tabular}{ | c | c | c | c |  c | c | c | c | c | c |}
    \hline
    $M_S$ (GeV)& $\kappa(M_Z)$ & $\lambda_S(M_Z)$ & $g_1$ & $g_2$ & $g_3$ & $y_t$ & $\lambda$ & $\kappa$ & $\lambda_S$\\
\hline
    620 & 0.185 & 1 & 0.478 & 0.506 & 0.487   & 0.382 & $-0.0029$ & 0.424 &  4.66 \\
    \hline
    795 & 0.239 & 0.389 & 0.478 & 0.506 & 0.487 & 0.382 & 0 & 0.412 & 1  \\         \hline
    \end{tabular}
    \caption{\textit{ Values of all {\rm SM+}$S$ coupling constants at $\mpl  = 1.2 \times 10^{19}$~GeV with $M_t=173.1$~GeV, $M_h=125.7$~GeV and $\alpha_S(M_Z)=0.1184$.}}
    \label{table2Scalar}
\end{center}
\end{table}
%%%%%%%%%

For SM+$S$, the running~\ref{eq:betasinglet} depends on the extra parameters $M_S$, $\kappa(M_Z)$ and $\lambda_S(M_Z)$. Assuming the values of SM parameters at $M_t$ as given in eqns.~\ref{eq:g1mt}$-$ \ref{eq:lammt}, for two different sets of $M_S$, $\kappa(M_Z)$ and $\lambda_S(M_Z)$, the values of all parameters at $\mpl$ in SM+$S$ model in Table~\ref{table2Scalar} has been presented.
The first set stands for our benchmark point, as described later. For this choice, $\lambda(\mpl)$ is negative. The second set is chosen such that $\lambda(\mpl)=0$.
Note that as the running of new physics parameters is not considered till $M_S$, in this case it is all the same to specify these parameters either at $M_Z$ or at $M_t$. 

In the SM, the gauge couplings $g_1,g_2,g_3$, top Yukawa coupling $y_t$ do not vanish at $\mpl$. The same is true in SM+$S$ model~\cite{Gabrielli:2013hma}, since running of these couplings are hardly affected by $S$, as displayed in Fig.~\ref{fig:SMScalar}.  Higgs portal coupling $\kappa$ and scalar self-quartic coupling $\lambda_S$ increase with energy. The rise of $\lambda_S$ is so rapid that it may render the theory nonperturbative at higher energies. For example, if $\lambda_S(M_Z)>1.3$, $\lambda_S$ becomes nonperturbative before $\mpl$.  Higgs self-quartic coupling $\lambda$ also gets affected by inclusion of $S$. But  the change is not visible in Fig.~\ref{fig:SMScalar}. 
%%%%RGE RUNNING
 \begin{figure}[h!]
 \begin{center}
 % \subfigure[]{
 \includegraphics[width=3.7in,height=3.1in, angle=0]{./scalar/CouplingSMScalar}
 \caption{\label{fig:SMScalar} \textit{  {\rm SM+}$S$ RG evolution of the gauge couplings $g_1,g_2,g_3$, top Yukawa coupling $y_t$, Higgs self-quartic coupling $\lambda$, Higgs portal coupling $\kappa$ and scalar self-quartic coupling $\lambda_S$ in $\MS$ scheme. } }
 \end{center}
 \end{figure}
%%%%RGE RUNNING
%%%%%
%%%%lam running
 \begin{figure}[h!]
 \begin{center}
 {\includegraphics[width=2.7in,height=2.7in, angle=0]{./scalar/LambdaSMScalar}}
 \caption{\label{fig:lambda} \textit{ RG evolution of $\lambda$ in the {\rm SM+}$S$ for our benchmark point. $3\sigma$ bands for $M_t,M_h$ and $\alpha_s(M_Z)$ are displayed.} }
 \end{center}
 \end{figure}
%%%%lam running

As the issue of stability hinges on the value of $\lambda$ at higher energies, the running of $\lambda$ is focused for SM+$S$ model in Fig.~\ref{fig:lambda} as for the SM in Fig.~\ref{fig:couplings}(b), for a {\em benchmark point}  $M_S = 620$ GeV, $\kappa(M_Z)=0.185$ and $\lambda_S (M_Z)=1$.
It has been observed that the behavior of $\lambda$ running might change significantly, modifying instability scale $\Lambda_I$ to $1.68 \times 10^{11}$~GeV, whereas in SM $\Lambda_I\sim 1.9 \times 10^{10}$ GeV (see eqn.~\ref{eq:instbilscaleSM}).
It has the potential to push out the EW vacuum from metastability to a stable vacuum.
The benchmark point was chosen keeping in mind that the new physics effects are clearly visible, yet the vacuum is still in metastable state.
This point also satisfies the WMAP and Planck imposed DM relic density constraint $\Omega h^2=0.1198\pm 0.0026$~\cite{Ade:2013zuv}. 
%%%%lambda effective
 \begin{figure}[h!]
 \begin{center}
 \subfigure[]{
 \includegraphics[width=2.7in,height=2.7in, angle=0]{./scalar/Effectivelambda_dark}}
 %\hskip 15pt
 \subfigure[]{
 \includegraphics[width=2.7in,height=2.7in, angle=0]{./scalar/LambdavsDarkMass}}
 \caption{\label{fig:lambdaef} \textit{$({\bf a})$ RG evolution of $\lambda$ (red band), $\lambda _{\rm eff}$ (blue band)  and  $\beta_\lambda$ (dot-dashed black) in {\rm SM+}$S$ for our benchmark point. $({\bf b})$~Evolution of  $\lambda$ for different $\kappa(M_Z)$. Each $\kappa(M_Z)$ corresponds to a specific $M_S$ to satisfy DM relic density $\Omega h^2 \approx$ 0.1198.} }
 \end{center}
 \end{figure}
%%%%lambda effective

As defined in eqn.~\ref{lameffscalar}, $\lambda_{\rm eff}$ differs from $\lambda$ as it takes care of loop corrections. In the SM, in Fig.~\ref{fig:lambdaSM}, one can see that the difference $\lambda_{\rm eff}-\lambda$ is always positive and negligible near $\mpl$. Similar features has also been seen in {\rm SM+}$S$ model (see Fig.~\ref{fig:lambdaef}(a)).
However, the instability scale $\Lambda_I$ changes significantly if $\lambda_{\rm eff}$ instead of $\lambda$ is chosen to work: In SM, the instability scale changes to $1.25 \times 10^{11}$~GeV and in {SM+}$S$, it becomes $1.7\times 10^{12}$~GeV.
Also $\beta_\lambda$ has been plotted to show that at high energies, $\lambda$, $\lambda_{\rm eff}$ and $\beta_\lambda$ all seem to vanish. 

In Fig.~\ref{fig:lambdaef}(b) the RGE running of $\lambda$ for various new physics parameters has been displayed to explicitly demonstrate that as $\kappa(M_Z)$ increases, for a given energy, $\lambda$ assumes a higher value~\cite{Kadastik:2011aa,Chen:2012faa}.
Finally, for some parameter space, $\lambda$ never turns negative, implying stability of the EW vacuum. It happens due to the $\kappa^2/2$ term in $\beta_\lambda$.  Due to this positive contribution, the presence of the scalar never drives EW vacuum towards instability.
Next, the tunneling probability will be calculated to demonstrate stability issues with EW vacuum in this model SM+$S$.
%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Tunneling probability and Metastability in SM+$S$}
\label{chapt3}
The present data on $M_h$ and $M_t$ indicate that the Universe might be residing in a false vacuum in SM, waiting for a quantum tunneling to a true vacuum lying close to the Planck scale. 

The vacuum decay probability ${\cal P}_0$ of EW vacuum at the present epoch is given in eqn.~\ref{prob}. In $S(\Lambda_B)=\frac{8\pi^2}{3|\lambda(\Lambda_B)|}$, the effective Higgs quartic coupling as given in eqn.~\ref{lameffscalar} has been used.
 %%%%tunneling probability
 \begin{figure}[h!]
 \begin{center}
\subfigure[]{
 \includegraphics[width=2.7in,height=2.7in, angle=0]{./scalar/tunnelingprob}}
 %\hskip 15pt
 \subfigure[]{
 \includegraphics[width=2.7in,height=2.7in, angle=0]{./scalar/tunnelingvskappaplots}}
 \caption{\label{fig:TunS} \textit{ $({\bf a})$ Tunneling probability ${\cal P}_0$ as a function of  $M_t$. The left band corresponds to {\rm SM} and the right one to {\rm SM+}$S$ for our benchmark point. Light-green band stands for $M_t$ at $\pm 1\sigma$. $({\bf b})$ ${\cal P}_0$ as a function of $\kappa(M_Z)$ for various $\lambda_S(M_Z)$.} }
 \end{center}
 \end{figure}
  %%%%tunneling probability
The metastability and perturvativity constraints in this model are shown here.

\begin{itemize}
\item
If $\lambda(\Lambda_B)>\frac{4\pi}{3}$, $|\kappa|>8\pi$, $|\lambda_S| > 8\pi$, then the theory is nonperturbative. 
\item
If $\lambda(\Lambda_B)>0$, then the vacuum is stable. 
\item
If $0>\lambda(\Lambda_B)>\lambda_{\rm min}(\Lambda_B)$, then the vacuum is metastable. 
\item
If $\lambda(\Lambda_B)<\lambda_{\rm min}(\Lambda_B)$, then the vacuum is unstable. 
\item
If $\lambda_S<0$, the potential is unbounded from below along the $S$-direction. 
\item
If $\kappa<0$, the potential is unbounded from below along a direction in between $S$ and $H$.  
\end{itemize}
In Fig.~\ref{fig:TunS} tunneling probability ${\cal P}_0$ as a function of  $M_t$ has been plotted. To calculate ${\cal P}_0$, the minimum value of $\lambda_{\rm eff}$ (see eqn.~\ref{lameffscalar}) has been found and put the same in $S(\Lambda_B)$. The right band corresponds to the tunneling probability for our benchmark point. 
For comparison, the same plot for SM as the left band in Fig.~\ref{fig:TunS}(a) is shown. 1$\sigma$ error bands in $\alpha_S$ and in $M_h$ are also displayed. The error due to $\alpha_S$ is clearly more significant than that due to $M_h$.
It has been observed that for a given $M_t$, these new physics effects lower the tunneling probability. It bolsters our earlier observation that scalar $S$ helps the EW vacuum to come out of metastability.
It has been demonstrated in Fig.~\ref{fig:TunS}(b), where 
${\cal P}_0$ as a function of $\kappa(M_Z)$ for different choices of $\lambda_S(M_Z)$ has been plotted, assuming central values for $M_h$, $M_t$ and $\alpha_S$. It has been seen that for low values of $\kappa(M_Z)$, ${\cal P}_0$ tends to coincide with its SM value. For a given $\kappa(M_Z)$, for higher $\lambda_S(M_Z)$, ${\cal P}_0$ gets smaller, making the EW vacuum more stable.

\subsection{Phase diagrams in SM+$S$}
\label{chapt4}
The phase diagrams in different parameter planes for this model has been presented to demonstrate the stability of the EW vacuum.
 
%%%%mtmhphase
 \begin{figure}[h!]
 \begin{center}
 \subfigure[]{
 \includegraphics[width=2.7in,height=2.7in, angle=0]{./scalar/MtMh}}
 %\hskip 15pt
 \subfigure[]{
 \includegraphics[width=2.7in,height=2.7in, angle=0]{./scalar/MhMtpurt}}
 \caption{\label{fig:Mt_MhScalar} \textit{$({\bf a})$ In {\rm SM+}$S$, regions of absolute stability~(green), metastability~(yellow), instability~(red) of the EW vacuum in the $M_h - M_t$ plane phase diagram is presented for the benchmark point $M_S = 620$~GeV, $\kappa(M_Z)=0.185$ and $\lambda_S (M_Z)=1$. 
 $({\bf b})$ Similar plot for $M_S = 360$~GeV, $\kappa(M_Z)= 0.105$ and $\lambda_S (M_Z) = 1.6$. The orange region  corresponds to nonperturbative zone for $\lambda_S$.
The three boundary lines (dotted, solid and dotted red) correspond to $\alpha_s(M_Z)=0.1184 \pm 0.0007$. The gray areas denote the experimentally favored zones for $M_h$ and $M_t$ at $1$, $2$ and  $3\sigma$. } }
 \end{center}
 \end{figure}
%%%%mtmhphase

%%%%Mt-alphaS phase diagram
 \begin{figure}[h!]
 \begin{center}
 {\vspace{-0.2cm}
 \includegraphics[width=3in,height=2.7in, angle=0]{./scalar/alphavsmtplots}}
 \caption{\label{fig:Alpha_MtScalar} \textit{Phase diagram in $M_t-\alpha_S(M_Z)$ plane in {\rm SM+}$S$ model for our benchmark point. Regions of absolute stability~(green), metastability~(yellow), instability~(red) of the EW vacuum are marked. The dotted lines correspond to $\pm 3\sigma$ variation in $M_h$ and the gray areas denote the experimental allowed region for $M_t$ and $\alpha_S(M_Z)$ at $1$, $2$ and  $3\sigma$.} }
 \end{center}
 \end{figure}
%%%%Mt-alphaS phase diagram 
In the SM, the phase diagram in $M_h-M_t$ plane is given in Fig.~\ref{fig:Mt_MhSM}. Given the measured errors on $M_t$ and $M_h$, the SM phase diagram indicates that the stability of EW vacuum is excluded\footnote{In a mass dependent renormalization scheme, such exclusion happens at $3.5\sigma$~\cite{Spencer-Smith:2014woa}.} at $\sim 3\sigma$. However, the extra scalar in this model modifies these findings, as illustrate by
the phase diagram in the $M_h - M_t$ plane for SM+$S$ in Fig.~\ref{fig:Mt_MhScalar}. For our benchmark point, it has been seen that the boundaries shift towards higher values of $M_t$, so that the EW vacuum stability is excluded only at 1.1$\sigma$, indicated by the blue-dashed ellipse.
For  $M_S = 360$~GeV, $\kappa(M_Z)= 0.105$ and $\lambda_S(M_Z) = 1.6$, the plot is redrawn to highlight the fact that $\lambda_S$ might turn out to be too large, so that the theory becomes nonperturbative (marked as the orange region in Fig.~\ref{fig:Mt_MhScalar}(b)).
Here EW vacuum stability is excluded at 2$\sigma$. All these boundaries separating various stability regions in the phase diagram depend on $\alpha_S$. 1$\sigma$ bands for the same is also displayed in these figures.

Given the sizable error on $\alpha_S(M_Z)$, it is instructive to draw the phase diagram in the $M_t-\alpha_S(M_Z)$ plane as well. This diagram for SM is available in Fig.~\ref{fig:alpha-mt}. The same is presented in Fig.~\ref{fig:Alpha_MtScalar} for this model using our benchmark point. With increase of $\kappa(M_Z)$ and/or $\lambda_S(M_Z)$, the boundaries between different stability regions shift towards right, allowing the EW vacuum to be more stable.

%%%%constraints1
 \begin{figure}[h!]
 \begin{center}
% \subfigure[]{
 \includegraphics[width=3in,height=2.7in, angle=0]{./scalar/kappaMs}
 \caption{\label{fig:Mskappa} \textit{ Phase diagram in $\kappa(M_Z)-M_S$ plane in {\rm SM+}$S$. Regions of absolute stability (green), metastability (yellow) of the EW vacuum for $\lambda_S (M_Z) = 1$ are shown. The red solid line corresponds to $\Omega h^2 \approx$ 0.1198. The red dashed lines correspond to 3$\sigma$ error on $\Omega h^2$.} }
 \end{center}
 \end{figure}
%%%%constraints1

The phase diagram for $\kappa(M_Z)-M_S$ plane is displayed in Fig.~\ref{fig:Mskappa}. As addition of the scalar does not drive the EW vacuum towards instability, there is no unstable region marked on the plot.
Between the dashed lines, the allowed region is marked ensuing from relic density constraints. 

In SM, the vacuum stability, metastability and perturbativity bound are given in eqns.~\ref{MassMh}$-$ \ref{MassMhpert}.
In SM+$S$ model, change in $M_h$ bounds with respect to $\kappa(M_Z)$ was considered in Refs.~\cite{Gonderinger:2009jp, Eichhorn:2014qka} for different cut-off scales, considering stability aspects only.
As shown in Fig.~\ref{fig:Mhkappa}, in presence of the scalar $S$, these bounds shift to lower values for larger $\kappa(M_Z)$.
For large values of $\kappa(M_Z)$, depending on the choice of $\lambda_S$ at $M_Z$, $\lambda_S(\mpl)$ may become so large that the theory becomes nonperturbative.
This imposes further constraints on the parameter space, shown as the curved line representing $\lambda_S(\mpl)=8\pi$. As before, for a given $\kappa(M_Z)$, $M_S$ is chosen in such a way that  $\Omega h^2\approx 0.1198$ for $M_h=125.7$~GeV. However, in the plot, as $M_h$ changes, $\Omega h^2$ also changes. But this variation is contained within 3$\sigma$. 
%%%%kappaMH phase
 \begin{figure}[h!]
 \begin{center}
% \subfigure[]{
 \includegraphics[width=3.3in,height=2.7in, angle=0]{./scalar/mhkappaplot}
 \caption{\label{fig:Mhkappa} \textit{ Phase diagram in $\kappa(M_Z)- M_h$ plane in {\rm SM+}$S$. Regions of absolute stability (green), metastability (yellow) and instability (red) of the EW vacuum for $\lambda_S (M_Z) = 1$ are displayed. $\lambda$ and/or $\lambda_S$ are/is nonperturbative in the orange region. The blue dashed line corresponds to $M_h=125.7$~GeV. } }
 \end{center}
 \end{figure}
%%%%kappaMH phase
\subsection{Confidence level of vacuum stability in SM+$S$}
%%%%%%%%%%%%%%%%%%%%%
As new physics effects do change the stability of EW vacuum, it is important to show the change in the confidence level at which stability is excluded or allowed.
In Fig.~\ref{fig:kappaconfidence}, the confidence level against $\kappa(M_Z)$ has been plotted for $M_t=173.1$~GeV, $M_h=125.7$~GeV and $\alpha_S(M_Z)=0.1184$. $M_S$ is dictated by $\kappa(M_Z)$ to satisfy $\Omega h^2\approx 0.1198$.
For $\lambda_S(M_Z)=1$, It has been seen that the EW vacuum becomes stable for  $\kappa(M_Z)=0.24$ onward. For a lower $\lambda_S(M_Z)$, this point shifts to a higher value. If $\lambda_S(M_Z)=0$, stability is assured for $\kappa(M_Z)\ge 0.27$. Note that as $\kappa$ dependence in RGE running of $\lambda$ creeps in through the term $\kappa^2/2$ in $\beta_\lambda$, the stability strongly depends on $\kappa(M_Z)$. However, as  $\beta_\lambda$ depends on $\lambda_S$ only {\it via} $\kappa$ running, although $\lambda_S$ running is relatively strong, the stability of EW vacuum does not change appreciably when $\lambda_S(M_Z)$ is varied from $0$ to $1$.

%%%%confidence
 \begin{figure}[h!]
 \begin{center}
 {
 \includegraphics[width=3in,height=2.7in, angle=0]{./scalar/kavsconfdncplot}}
 \caption{\label{fig:kappaconfidence} \textit{ Dependence of confidence level (one-sided) at which EW vacuum stability is excluded/allowed on $\kappa(M_Z)$ in {\rm SM+}$S$. Regions of absolute stability (green) and metastability (yellow) of EW vacuum are shown.} }
 \end{center}
 \end{figure}
%%%%confidence
%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Asymptotic safety in SM+$S$}
%%%%asymptotic safety
 \begin{figure}[h!]
 \begin{center}
 \subfigure[]{
 \includegraphics[width=2.7in,height=2.7in, angle=0]{./scalar/MtMhPlanck}}
 %\hskip 15pt
 \subfigure[]{
 \includegraphics[width=2.7in,height=2.7in, angle=0]{./scalar/mtmh10power14}}
 \caption{\label{fig:asymp} In {\rm SM+}$S$ model, \textit{$({\bf a})$ Contour plot for $\lambda(\mpl) =0$ (red line) and  $\beta_{\lambda}(\mpl)=0$ (blue line) for our benchmark point. $({\bf b})$ Similar plot for $\lambda ({\Lambda}) =0$ and  $\beta_{\lambda}(\Lambda)=0$, where $\Lambda=3.8\times10^{14}$~GeV. Dotted lines correspond to $\pm 3\sigma$ variation in $\alpha_s(M_Z)$. The gray areas denote the experimental allowed region for $M_h$ and $M_t$ at $1$, $2$ and  $3\sigma$.} }
 \end{center}
 \end{figure}
%%%%asymptotic safety

Shaposhnikov and Wetterich predicted~\cite{Shaposhnikov:2009pv} mass of the Higgs boson of $126$~GeV imposing the constraint $\lambda(\mpl)=\beta_{\lambda}(\mpl)=0$, in a scenario known as asymptotic safety of gravity. As mentioned before, this corresponds to two degenerate vacua. In Fig.~\ref{fig:lambetampl}, it has been shown that the present error in $M_t$ and $M_h$ does not allow this condition to be realised in SM. In SM+$S$ model, the situation worsens~\cite{Haba:2013lga} and it has  demonstrated in Fig.~\ref{fig:asymp}(a) for our benchmark point. In presence of the scalar, the values of $M_t$ and $M_h$, required to satisfy this condition, are pushed far away from the experimentally favored numbers: For our benchmark point this condition is satisfied at  $M_h=140.8$ GeV and  $M_t=179.5$ GeV.

However, it is possible to meet this condition at a lower energy than at $\mpl$. In Fig.~\ref{fig:asymp}(b), it is demonstrated that at a different point in the parameter space: $M_S = 914$~GeV, $\kappa(M_Z)=0.276$ and $\lambda_S (M_Z)=0.229$, the condition $\lambda ({\Lambda}) =\beta_{\lambda}(\Lambda)=0$ is indeed satisfied at $\Lambda=3.8\times10^{14}$ GeV and is also consistent with experimentally allowed range for $M_t$ and $M_h$. The value of $\Lambda$ decreases with  $\lambda_S (M_Z)$ and $\kappa(M_Z)$. The corresponding value of $M_S$ is chosen to satisfy relic density of DM constraints. 
Also, it is difficult to simultaneously satisfy Veltman condition at $\mpl$~\cite{Haba:2013lga}. All these observations indicate that some new physics could be operational at very high energies  to take care of such issues.

\section{Doublet scalar extension of SM}\label{doubletexten}
The model is popularly known in the literature as the inert doublet~(ID) model, first proposed by Deshpande and Ma~\cite{Deshpande:1977rw}. 

In previous Section~\ref{SingletSMext}, stability analysis, including NNLO corrections, has done for extended singlet scalar DM model. The stability of the EW vacuum was shown to depend on new physics parameters. 
In this section such an analysis has been extended to the ID model. It has been assumed that ID DM is the only DM particle which saturates the entire DM relic density. In this context, the constraints on the parameters of the ID model have been reviewed. 


A detailed study on the ID parameter space was performed in Refs.~\cite{Dolle:2009fn, Gustafsson:2012aj,Honorez:2010re,Goudelis:2013uca, Arhrib:2013ela,Chakrabarty:2015yia,Hambye:2007vf,Coleman:1973jx,Chakrabarty:2014aya, Das:2015mwa} indicating bounds from absolute EW vacuum stability, perturbativity, collider study, EW precision tests (EWPT), etc.
In this work~\cite{Khan:2015ipa}, the new parameter spaces have been found allowing the metastability of the Higgs potential.

\subsection{Inert Doublet Model}
\label{sec:IDM}
In this model, the standard model is extended by adding an extra ${ SU(2)_L}$ doublet scalar, odd under an additional discrete $Z_2$ symmetry. The $Z_2$ symmetry prohibits the inert doublet to acquire a vacuum expectation value.

The scalar potential of eqn.~\ref{pot} at the tree level with exact $Z_2$ symmetry, is given\footnote{Here the notation of Higgs quartic coupling $\lambda_1$ is used instead of $\lambda$.} by,
%%%%%%%%%%%%%%%%%%
\begp
\allowdisplaybreaks \bea
V(\Phi_1,\Phi_2) &=& m_{11}^2 |\Phi_1|^2 + \lambda_1 |\Phi_1|^4+ m_{22}^2 |\Phi_2|^2 + \lambda_2 |\Phi_2|^4\nn\\
&&+ \lambda_3 |\Phi_1|^2 |\Phi_2|^2 
+  \lambda_4 |\Phi_1^\dagger \Phi_2|^2 + \frac{\lambda_5}{2} \left[ (\Phi_1^\dagger \Phi_2)^2 + { h.c.}\right]  \, ,
\label{Scalarpot}
\eea
\eegp
%%%%%%%%%%%%%%%%%%%%
where the SM Higgs doublet $\Phi_1$ and the inert doublet $\Phi_2$ are given by
%%%%%%%%%%%%%%%%%
%\renewcommand*{\arraystretch}{0}{
\begp
\allowdisplaybreaks \beq
	\Phi_1 ~=~ \left( \begin{array}{c} G^+ \\ \frac{1}{\sqrt{2}}\left(v+h+i G^0\right) \end{array} \right),
	\qquad
	\Phi_2 ~=~ \left( \begin{array}{c} H^+\\ \frac{1}{\sqrt{2}}\left(H+i A\right) \end{array} \right) \, \nn.
\eeq
\eegp
%%%%%%%%%%%%%%%%%%%%
$\Phi_2$ contains a $CP$ even neutral scalar $H$, a $CP$ odd neutral scalar $A$, and a pair of charged scalar fields $H^\pm$. The $Z_2$ symmetry prohibits these particles to decay entirely to SM particles. The lightest of $H$ and $A$ can then serve as a DM candidate. 

After EW symmetry breaking, the scalar potential is given by
%%%%%%%%%%%%%%%%%%
\begp
\allowdisplaybreaks \bea
V(h, H,A,H^\pm) &=&  \frac{1}{4} \left[ 2 m_{11}^2 (h+v)^2 + \lambda_1 (h+v)^4 +2 m_{22}^2 (A^2+H^2+2 H^+ H^-) \right. \nn \\
&& \left. + \lambda_2 (A^2 + H^2 + 2 H^+ H^-)^2  \right] \nn \\
&& + \frac{1}{2} (h+v)^2 \left[  \lambda_3 H^+ H^- 
+  \lambda_S  A^2  
+  \lambda_L  H^2 \right] \label{Scalarpot2}
\eea
\eegp
%%%%%%%%%%%%%%%%%%%%
where,
%%%%%%%%%%%%%%%%%%
\begp
\allowdisplaybreaks \bea
\lambda_{L,S}&=&\frac{1}{2}\left(\lambda_3+\lambda_4\pm\lambda_5\right) \, .
\eea
\eegp
%%%%%%%%%%%%%%%%%%%%
Masses of these scalars are given by,
%%%%%%%%%%%%%%%%
\begp
\allowdisplaybreaks \begin{align}
	M_{h}^2 &= m_{11}^2 + 3 \lambda_1 v^2,\nn \\
	M_{H}^2 &= m_{22}^2 +  \lambda_L v^2, \nn \\
	M_{A}^2 &= m_{22}^2 + \lambda_S v^2,\nn \\
	M_{H^\pm}^2 &= m_{22}^2 + \frac{1}{2} \lambda_3 v^2  \,\nn .
\end{align}
\eegp
%%%%%%%%%%%%%%%
For  $\lambda_4-\lambda_5<0$ and $\lambda_5>0$~($\lambda_4+\lambda_5<0$ and $\lambda_5<0$), %implies that 
$A$~($H$) is the lightest $Z_2$ odd particle (LOP).
In this work, $A$ has been taken as the LOP and hence, as a viable DM candidate.
Choice of $H$ as LOP will lead to similar results. 

For large DM mass, $M_A\gg M_Z$, appropriate relic density of DM is obtained if $M_A$, $M_H$, and $M_{H^\pm}$ are nearly degenerate that will be explained latter. Hence, in anticipation, one can define,
%%%%%%%%%%%%%%%%%%
\begp
\allowdisplaybreaks \bea
	\Delta M_H&=& M_H-M_A, \nn\\
	\Delta M_{H^\pm}&=&M_{H^\pm}-M_A \nn\, .
\eea
\eegp
%%%%%%%%%%%%%%%%%%%%
so that the new independent parameters for the ID model become $\{M_A, \Delta M_H, \Delta M_{H^\pm},\\ \lambda_2, \lambda_S\}$. Here $\lambda_S$ is chosen as $A$ is treated as the DM particle.

The one-loop effective potential for $h$ in the $\MS$ scheme and the Landau gauge is given by   
%%%%%%%%%%%%%%%%%
\begp
\allowdisplaybreaks \beq
V_1^{{\rm SM}+{\rm ID}}(h)= V_1^{\rm SM}(h) + V_1^{\rm ID}(h)
\eeq
\eegp
%%%%%%%%%%%%%%%%%%%%
The SM one-loop effective Higgs potential $V_1^{\rm SM}(h)$ can be found in eqn.~\ref{V1loop} and the additional contribution to the one-loop effective potential due to the inert doublet is given by~\cite{Hambye:2007vf}
%%%%%%%%%%%%%%%%%
\begp
\allowdisplaybreaks \beq
V_1^{\rm ID}(h)= \sum_{j=H,A,H^+,H^-} \frac{1}{64 \pi^2} M_j^4(h) \left[ \ln\left(\frac{M_j^2(h)}{\mu^2(t)} \right)- \frac{3}{2} \right] 
\eeq
\eegp
%%%%%%%%%%%%%%%%%%%%
where, 
%%%%%%%%%%%%%%%%%
\begp
\allowdisplaybreaks \beq
M_j^2(h)=\frac{1}{2} \,\lambda_{j}(t) \, h^2(t)+m_{22}^2(t) 
\eeq
\eegp
%%%%%%%%%%%%%%%%%%%%
with $\lambda_{A}(t)=2 \lambda_{S}(t)$, $\lambda_{H}(t)=2 \lambda_{L}(t)$, and $\lambda_{H^\pm}(t)= \lambda_{3}(t)$.

In the present work, in the Higgs effective potential, SM contributions are taken at the two-loop level, whereas the ID scalar contributions are considered at one loop only. 

For $h \gg v$, the Higgs effective potential can be approximated as
%%%%%%%%%%%%%%%%%
\begp
\allowdisplaybreaks \beq
V_{\rm eff}^{{\rm SM}+{\rm ID}}(h) \simeq \lambda_{\rm 1,eff}(h) \frac{h^4}{4}\, ,
\label{efflamID}
\eeq\eegp
%%%%%%%%%%%%%%%%%%%%
with
%%%%%%%%%%%%%%%%%
\begp
\allowdisplaybreaks \beq
\lambda_{\rm 1,eff}(h) = \lambda_{\rm 1,eff}^{\rm SM}(h) +\lambda_{\rm 1,eff}^{\rm ID}(h)\, ,
\label{lameffidm}
\eeq
\eegp
%%%%%%%%%%%%%%%%%%%%
where $\lambda_{\rm 1,eff}^{\rm SM}$ can be found in eqn.~\ref{eq:effqurtic} and,
%%%%%%%%%%%%%%%%%%
\begp
\allowdisplaybreaks \bea
 \lambda_{\rm 1,eff}^{\rm ID}(h)&=&\sum_{j=L,S,3} e^{4\Gamma(h)} \left[\frac{\delta_j \lambda_j^2}{64 \pi^2}  \left(\ln\left(\delta_j\lambda_j\right)-\frac{3}{2}\right ) \right]\, . 
 \label{efflamdoublet}
\eea
\eegp
%%%%%%%%%%%%%%%%%%%%
Here $\delta_j=1$ when $j=L,S$;  $\delta_j=\frac{1}{2}$ for $j=3$; and anomalous dimension $\gamma(\mu)$ of the Higgs field takes care of  its wave function renormalization (see the Appendix).
As quartic scalar interactions do not contribute to wave function renormalization at the one-loop level, ID does not alter  $\gamma(\mu)$ of the SM. All running coupling constants are evaluated at $\mu=h$.

If DM mass $M_A$ is larger than $M_t$, then the ID starts to contribute after the energy scale $M_A$. For  $M_A<M_t$, the contributions of ID to the $\beta$-functions (see eqns.~\ref{betal_1}$-$ \ref{betal_5}) are rather negligible for the running from $M_A$ to $M_t$, as is evident from the expressions.

To compute the RG evolution of all the couplings, all the couplings with threshold corrections at $M_t$ has been calculated. In Table~\ref{table1IDM} a specific set of values of $\lambda_i$ at $M_t=173.1$~GeV and at $\mpl = 1.2 \times 10^{19}$~GeV for $M_h=125.7$~GeV and $\alpha_s\left(M_Z\right)=0.1184$ have been provided. In Fig.~\ref{fig:SMIDM} the running of the scalar couplings $(\lambda_i)$ has been shown for this set of parameters. It has been seen that for this specific choice of parameters, $\lambda_1$ assumes a small negative value leading to a metastable EW vacuum as discussed in the following sections. This set is chosen to reproduce the DM relic density in the right ballpark.
%%%%%%%%%
%\renewcommand*{\arraystretch}{15}{
\setlength\tablinesep{2pt}
\begin{table}[h!]
\begin{center}
    \begin{tabular}{| c | c | c | c | c | c | c | c |}
    \hline
     &$\lambda_S$ & $\lambda_L$ & $\lambda_2$ & $\lambda_3$ & $\lambda_4$ & $\lambda_5$ & $\lambda_1$\\
\hline
   ~$M_{t}$ ~&~ 0.001 ~&~ 0.039 ~&~ 0.10 ~&~ 0.0399 ~&~ 0.00003   ~&~ 0.038 ~&~ 0.127~\\
            \hline
   $\mpl$ & 0.046 & 0.082 & 0.127 & 0.090 & 0.038   & 0.036 & $-0.009$\\
              \hline
    \end{tabular}
    \caption{A set of values of all ID model coupling constants at  $M_t$ and $\mpl$ for $M_{A}=573$ GeV, $\Delta M_{H^\pm}=1$ GeV, $\Delta M_{H}=2$ GeV, and $\lambda_S\left(M_Z\right)=0.001$.}
    \label{table1IDM}
\end{center}
\end{table}
%%%%%%%%%
\subsection{Constraints on ID model}
\label{sec:constraintsID}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
ID model parameter space is constrained from theoretical considerations like  absolute vacuum stability, perturbativity and unitarity of the scattering matrix.  EW precision measurements and direct search limits at LEP, LHC put severe restrictions on the model. The recent measurements of Higgs decay width at the LHC put additional constraints. The requirement that the ID DM saturates the DM relic density all alone restricts the allowed parameter space considerably. The tree level vacuum stability bound of the ID model can be found in eqn.~\ref{stabilitybound}. The unitary (eqn.~\ref{unitary}) and perterbativity (eqn.~\ref{pertIDM}) bounds up to the  $\mpl$ have also been taken into account.
%%%%RGE RUNNING
 \begin{figure}[h!]
 \begin{center}
 % \subfigure[]{
 \includegraphics[width=3.1in,height=2.7in, angle=0]{./Plots/couplingvsenergy}
 \caption{\label{fig:SMIDM} \textit{ {\rm IDM} RG evolution of the couplings $\lambda_i\left(i=1,..,5\right), \lambda_L, \lambda_S$ for the set of parameters in Table~\ref{table1IDM}. } }
 \end{center}
 \end{figure}
%%%%RGE RUNNING
%%%%%%%%%%%%%%%%%%%%
\subsubsection{Bounds from electroweak precision experiments}
%%%%%%%%%%%%%%%%%%%%%%
Bounds ensuing from electroweak precision experiments are imposed on new physics models {\it via} Peskin-Takeuchi~\cite{Peskin:1991sw} $S,~ T,~ U$ parameters. The additional contributions from 2HDM can be found in eqn.~\ref{STU2HDM}, which are modified for ID model~\cite{Barbieri:2006dq,Arhrib:2012ia} as,
%%%%%%%%%%%%%%%%%%
\begp
\allowdisplaybreaks \bea
 \Delta S &=& \frac{1}{2\pi}\Bigg[ \frac{1}{6}\ln\left(\frac{M^2_{H}}{M^2_{H^\pm}}\right) -
  \frac{5}{36} + \frac{M^2_{H} M^2_{A}}{3(M^2_{A}-M^2_{H})^2} + 
\frac{M^4_{A} (M^2_{A}-3M^2_{H})}{6(M^2_{A}-M^2_{H})^3} \ln \left(\frac{M^2_{A}}{M^2_{H}}\right)\Bigg], \nn\\
 \Delta T &=& \frac{1}{32\pi^2 \alpha v^2}\Bigg[ F\left(M^2_{H^\pm}, M^2_{A}\right)
+ F\left(M^2_{H^\pm}, M^2_{H}\right) - F\left(M^2_{A}, M^2_{H}\right)\Bigg]
\label{STparam}
\eea
\eegp
%%%%%%%%%%%%%%%%%%%%
The NNLO global electroweak fit results of $\Delta S$, $\Delta T$ and $\Delta U$ are given eqn.~\ref{STU1} have been used, with a correlation coefficient of $+0.91$, fixing $\Delta U$ to zero. The contribution of the scalars in the ID model to $\Delta U$ is rather negligible. 
%%%%ContourSTU
 \begin{figure}[h!]
 \begin{center}
% \subfigure[]{
 \includegraphics[width=2.7in,height=2.7in, angle=0]{./Plots/STUCheckplotnew11}
  \caption{\label{fig:STUcheck} \textit{Allowed parameter space in $\Delta M_{H^\pm}-\Delta M_{H}$ plane for $M_A=70$~GeV and $\lambda_S=0.007$ in {\rm IDM}. Constraints from $S$ and $T$ parameters are shown by solid black, green and red lines. The blue band corresponds the 3$\sigma$ variation in $\Omega h^2=0.1198\pm0.0026$~\cite{Ade:2013zuv}. On the brown region the unitarity bound is violated on or before $\mpl$. The cross-hatched region is excluded from LEP\,II data. }} 
 \end{center}
 \end{figure} 
%%%%ContourSTU
To assess the implications of $S$ and $T$ constraints on the ID model, in Fig.~\ref{fig:STUcheck}, in the $\Delta M_{H^\pm}-\Delta M_{H}$ plane, various constraints is displayed for $M_A=70$~GeV and $\lambda_S=0.007$.
This is the maximum value of $\lambda_S$ for the given DM mass, allowed by LUX~\cite{Akerib:2013tjd} direct detection data at 1$\sigma$.  The blue region allowed by relic density constraints shifts upwards for smaller $\lambda_S$.
Constraints on $\Delta S$ and $\Delta T$, as mentioned in eqn.~\ref{STU1}, are marked as black, green, and red  solid lines.
It has been seen that the $1\sigma$ bound on $\Delta T$ is the most stringent one. The black line corresponding to the lower limit on $\Delta S$ at $1\sigma$ can also be interesting. But the LEP\,II bounds, represented by the cross-hatched bar, take away a considerable part.
The line representing the $\Delta S$ upper limit is beyond the region considered and lies towards the bottom-right corner of the plot.
In this plot, increasing $M_H$ enhances $S$, but $T$ gets reduced.
In addition, if one demand unitarity constraints to be respected up to $\mpl$, assuming no other new physics shows up in between, the parameter space gets severely restricted.
In this plot, a small window is allowed by $\Delta T$ only at $2\sigma$, which satisfies DM relic density constraints. As mentioned earlier, this window gets further reduced with smaller $\lambda_S$ (the relic density band takes an ``L'' shape as shown in Fig.~\ref{fig:STU2}). 
\subsubsection{Direct search limits from LEP and LHC}
The decays $Z\ra AH$, $Z\ra H^+ H^-$, $W^\pm\ra A H^\pm$, and $W^\pm\ra H H^\pm$ are restricted from $Z$ and $W^\pm$ decay widths at LEP. It implies $M_{A} + M_{H} \geq M_{Z}$, $2M_{H^\pm}\geq M_{Z}$, and $M_{H^\pm} + M_{H,A} \geq M_{W}$. More constraints on the ID model can be extracted from chargino~\cite{Pierce:2007ut} and neutralino~\cite{Lundstrom:2008ai} search results at LEP\,II: The charged Higgs mass $M_{H^\pm}\geq 70$~GeV. The bound on $M_A$ is rather involved: If  $M_A<80$ GeV, then $\Delta M_H$ should be less than $\sim 8$ GeV, or else $M_H$ should be greater than $\sim 110$~GeV ({see Fig.~\ref{fig:STU1}}).
The Run 1 of LHC data provide significant constraints on the ID parameter space through the direct searches in final states with two leptons plus missing transverse energy~\cite{Belanger:2015kga}.
These analyses exclude inert scalar masses of up to about 55 GeV. For $M_{H^\pm}=85$ GeV and $M_{A}=55$ GeV, the $M_{H}\lesssim 145$ GeV are excluded at 4$\sigma$ and for $M_{A}>60$ GeV all masses of $H$ are allowed.
For $M_{H^\pm}>150$ GeV with $M_{A}=55$ GeV, $115\lesssim M_{H} \lesssim 160$ GeV region is excluded and $M_{A}>80$ GeV all masses of $H$ are allowed.
%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Bounds from LHC diphoton signal strength}
In the ID model, Higgs to diphoton signal strength $\mu_{\gamma\gamma}$ is defined as 
%%%%%%%%%%%%%%%%%
\begp
\allowdisplaybreaks \beq
\mu_{\gamma\gamma} = \frac{\sigma(gg\ra h\ra\gamma\gamma)}{\sigma(gg\ra h\ra\gamma\gamma)_{\rm SM}}\approx \frac{Br(h \rightarrow {\gamma\gamma})_{\rm ID}}{Br(h \rightarrow {\gamma\gamma})_{\rm SM}}
\eeq
\eegp
%%%%%%%%%%%%%%%%%%%%
using the narrow width approximation for the production cross-section of $\sigma(gg\ra h\ra \gamma\gamma)$ and the fact that $\sigma(gg\rightarrow h)$ in both the SM and ID are the same. 

Now if the ID particles have masses less than $M_h/2$, $h\rightarrow \rm ID,ID$ decays are allowed. In that case,
%%%%%%%%%%%%%%%%%
\begp
\allowdisplaybreaks \beq 
 \mu_{\gamma\gamma}= \frac{\Gamma(h\rightarrow \gamma\gamma)_{\rm ID}} {\Gamma(h\rightarrow \gamma\gamma)_{\rm SM}} ~ \frac{\Gamma_{\rm tot}(h\rightarrow \rm SM,SM)}{\Gamma_{\rm tot}(h\rightarrow {\rm SM,SM})+\Gamma_{{\rm tot}}(h \rightarrow {\rm ID,ID})}\, ,
 \label{mugagalow}
\eeq
\eegp
%%%%%%%%%%%%%%%%%%%%
where~\cite{Cao:2007rm} 
%%%%%%%%%%%%%%%%%
\begp
\allowdisplaybreaks \beq
\Gamma\left(h\rightarrow \rm ID,ID\right)= \frac{ v^2}{16\pi M_h }\lambda_{\rm ID}^2 \left(1-\frac{4 M_{\rm ID}^2}{M_{h}^2}\right)^{1/2}\, ,
\label{decaywidth}
\eeq
\eegp
%%%%%%%%%%%%%%%%%%%%
where for ${\rm ID}=A,H,H^\pm$, $\lambda_{\rm ID}=\lambda_S, \lambda_L, \sqrt{2}\,\lambda_3$.

In this case, the ID particles are heavier than $M_h/2$, 
%%%%%%%%%%%%%%%%%
\begp
\allowdisplaybreaks \beq 
 \mu_{\gamma\gamma}= \frac{\Gamma(h\rightarrow \gamma\gamma)_{\rm ID}}{\Gamma(h\rightarrow \gamma\gamma)_{\rm SM}}\, .
 \label{mugagahigh}
\eeq
\eegp
%%%%%%%%%%%%%%%%%%%%
In the ID model, the $H^\pm$ gives additional contributions at one loop. 
The analytical expression is given by~\cite{Djouadi:2005gj, Swiezewska:2012eh,Krawczyk:2013jta}
%%%%%%%%%%%%%%%%%
\begp
\allowdisplaybreaks \beq
\Gamma(h\rightarrow \gamma\gamma)_{\rm ID}=
\frac{\alpha^2 m_h^3}{ 256\pi^3
v^2}\left|\sum_{f}N^c_fQ_f^2y_f
F_{1/2}(\tau_f)+ y_WF_1(\tau_W)
+Q_{H^{\pm}}^2 \frac{v\mu_{{hH^+H^-}}}{
2m_{H^{\pm}}^2} F_0(\tau_{H^{\pm}})\right|^2\
\label{hgaga}
\eeq
\eegp
%%%%%%%%%%%%%%%%%%%%
where $\tau_i=m_h^2/4m_i^2$. $Q_{f}$, $Q_{H^{\pm}}$ denote electric charges of corresponding particles. $N_f^c$ is the color factor. $y_f$ and
$y_W$ denote Higgs couplings to $f\bar{f}$ and $WW$. $\mu_{hH^+H^-}= \lambda_3 v$ stands for the coupling constant of the $hH^+H^-$ vertex. The loop functions $F_{(0,\,1/2,\,1)}$  are defined as
%%%%%%%%%%%%%%%%%%
\begp
\allowdisplaybreaks \begin{align}
F_{0}(\tau)&=-[\tau-f(\tau)]\tau^{-2}\, ,\nn\\
F_{1/2}(\tau)&=2[\tau+(\tau-1)f(\tau)]\tau^{-2}\, ,\nn\\
F_{1}(\tau)&=-[2\tau^2+3\tau+3(2\tau-1)f(\tau)]\tau^{-2}\, , \nn
\label{loopfn}
\end{align}
\eegp
%%%%%%%%%%%%%%%%%%
where,
%%%%%%%%%%%%%%%%%
%\renewcommand*{\arraystretch}{0}{
\begp
\allowdisplaybreaks \beq
f(\tau)= \bigg\{\begin{array}{ll}
(\sin^{-1}\sqrt{\tau})^2\,,\hspace{60pt}& \tau\leq 1\\
-\frac{1}{ 4}[\ln{1+\frac{\sqrt{1-\tau^{-1}}}{1}-\sqrt{1-\tau^{-1}}}-i\pi]^2\,,\quad
&\tau>1
\label{ftau}
\end{array}\;,\;
\eeq
\eegp
%%%%%%%%%%%%%%%%%%%%
From the diphoton decay channel of the Higgs at the LHC, the measured values are  $\mu_{\gamma\gamma}$=$1.17\pm0.27$ from ATLAS~\cite{Aad:2014eha} and  $\mu_{\gamma\gamma}$=$1.14^{+0.26}_{-0.23}$ from CMS~\cite{Khachatryan:2014ira}. 

One can see that a positive $\lambda_3$ leads to a destructive interference between SM and ID contributions in eqn.~\ref{hgaga} and {\it vice versa}. Hence, for ID particles heavier than $M_h/2$, $\mu_{\gamma\gamma}<1$ ($\mu_{\gamma\gamma}>1$) when $\lambda_3$ is positive (negative). However, if these ID particles happen to be lighter than $M_h/2$, they might contribute to the invisible decay of the Higgs boson. Using the global fit result~\cite{Belanger:2013xza} that such an  invisible branching ratio is less than $\sim 20$\%, in eqn.~\ref{mugagalow}, the second ratio provides a suppression of $\sim 0.8$ -- $1$.

Now can negative $\lambda_3$ is allowed in the ID model? It will be discussed at the end of this section. 
The benchmark points with positive $\lambda_3$ is used here,
allowed at 1$\sigma$ by both CMS and ATLAS experiments. 

\subsubsection{Constraints from dark matter relic density and direct search limits}
As it has been seen that Higgs can decay to pair of inert particles (see eqns.~\ref{Scalarpot2},\ref{decaywidth}), so most of the parameter spaces with dark matter mass less than $M_h/2$, are strictly restricted from the Higgs invisible decay width of LHC and also from the direct detection experimental data. In this model the dark matter mass below 50 GeV are excluded from these constraints.
In Table~\ref{tableI1}, few benchmark points for IDM with the dark matter mass, $M_A(\equiv M_{DM})< M_h/2$ have been shown.

The heavy $CP$-even and charge Higgs mass have been fixed at 180 and 200 GeV respectively. The relic density, dark matter-nucleon cross-section, as well as the branching ratio of Higgs to pair of dark matter particles have been shown in the same table. For all these points, it has been seen that the dominant process in the dark matter annihilation is $AA\ra b \bar{b}$.
%%%%%%%%%%%%%%%%%%%
%\renewcommand*{\arraystretch}{15}{
\setlength\tablinesep{1pt}
\setlength\tabcolsep{6pt}
\begin{table}[h!]
\begin{center}
    \begin{tabular}{ | c | c |  c | c | c | c |}
    \hline
     $M_{DM}(\equiv M_A)$ (GeV) & $\lambda_S$ & Relic density &$\sigma_{SI}$ ${\rm ({cm}^2)}$& Br($h\rightarrow S S$) in $\%$\\
    \hline
     $54.7$ & 0.004 & 0.1263 & $1.78\times10^{-46}$ & 3.67   \\
     \hline
     $56$ & 0.0022 & 0.1197 & $3.47\times10^{-48}$ & 1.05   \\
     \hline
     $58.8$ & 0.0006 & 0.1222 & $2.4\times10^{-48}$ & 0.06   \\
     \hline
     $60$ & 0.00035 & 0.1236 & $1.13\times10^{-48}$ & 0.017   \\
     \hline
             \end{tabular}
    \caption{\textit{ Benchmark points with dark matter mass $M_{DM}< M_h/2$, with $M_{H^\pm}=200$ ${\rm GeV}$ and $M_{H^\pm}=180$ ${\rm GeV}$, which is allowed from the relic density constraint of WMAP and Planck, $\Omega h^2=0.1198\pm 0.0026$ within 3$\sigma$ confidence level, direct detection LUX (2013) and Higgs invisible decay width from the LHC. }}
    \label{tableI1}
\end{center}
\end{table}
%%%%%%%%%%%%%%%%%%

The ID dark matter candidate $A$ can self-annihilate into SM fermions. Once the DM mass is greater than the $W^\pm$-mass, so that the DM can annihilate into a pair of $W^\pm$ bosons, the cross-section increases significantly, thereby reducing DM relic density. Hence, it becomes difficult to saturate $\Omega h^2$ after $\sim 75$~GeV with positive $\lambda_S$, although for $M_A<75$~GeV, both signs of  $\lambda_S$ can be allowed to arrive at the right DM relic density $\Omega h^2$.

The role of the sign of $\lambda_S$ can be understood from the contributing diagrams to the  $AA\ra W^+ W^-$  annihilation processes. Four diagrams contribute: the $AAW^+ W^-$ vertex driven point interaction diagram (henceforth referred to as the $p$-channel diagram), $H^+$-mediated $t$- and $u$-channel diagrams, and the $h$-mediated $s$-channel diagram. For $AA\ra ZZ$  annihilation, the $t$- and $u$-channel diagrams are mediated by $H$. A negative $\lambda_S$ induces a destructive interference between the $s$-channel diagram with the rest, thereby suppressing $AA\ra W^+ W^-, ZZ$ processes. For DM masses of $75-100$~GeV, this can be used to get the appropriate $\Omega h^2$~\cite{Gustafsson:2012aj, LopezHonorez:2010tb}. To avoid large contributions from $t$- and $u$-channel diagrams and coannihilation diagrams, the values of $M_H$ and $M_{H^\pm}$ can be pushed to be rather large $\gtrsim 500$~GeV. However, to partially compensate the remaining $p$-channel diagram by the  $s$-channel one, $\lambda_S$ assumes a large negative value $\sim -0.1$, which is ruled out by the DM direct detection experiments. That is why in the ID model, DM can be realized below 75 GeV, a regime designated as the ``low'' DM mass region. 

%%%%
 \begin{figure}[h!]
 \begin{center}
 \subfigure[]{
 \includegraphics[width=2.7in,height=2.7in, angle=0]{./Plots/InertLowRelivsMDM}}
 %\hskip 15pt
 \subfigure[]{
 \includegraphics[width=2.7in,height=2.7in, angle=0]{./Plots/InertRelivsMDM}}
 \caption{\label{fig:relicvsmassIn} In {\rm IDM}, \textit{$({\bf a})$ Dark matter relic density $\Omega h^2$ as a function of the dark matter mass $M_{DM}(\equiv M_A)$ for different values of the Higgs portal coupling: $\lambda_S(M_Z)=0.002$ (black), $\lambda_S(M_Z)=0.005$ (brown), and $\lambda_S(M_Z)=0.008$ (red), with $\Delta M_{H^\pm}=\Delta M_{H}=50$ GeV. $({\bf b})$ For Higgs portal coupling: $\lambda_S(M_Z)=0.05$ (black), $\lambda_S(M_Z)=0.10$ (brown), and $\lambda_S(M_Z)=0.15$ (red), with $\Delta M_{H^\pm}=1$ GeV and $\Delta M_{H}=2$ GeV. The thin blue band corresponds to the relic density of the dark matter, $\Omega h^2=0.1198 \pm 0.0026$ (3$\sigma$) of the present the Universe. Light red band is disallowed from the Higgs invisible decay width.} }
 \end{center}
 \end{figure}
%%%%mtmhphase
%%%%%%%%%%%%%%%%%%%%
At ``high'' DM mass $M_A \gtrsim 500$~GeV, one can get the right $\Omega h^2$ due to a partial cancellation between different diagrams contributing to the $AA\ra W^+ W^-$ and $AA\ra ZZ$ annihilation processes. For example, in $AA\ra W^+ W^-$, the $p$-channel diagram tends to cancel with the $H^+$-mediated $t$- and $u$-channel diagrams~\cite{Hambye:2009pw, Goudelis:2013uca} in the limit $M_A\gg M_W$, and the sum of amplitudes of these diagrams in this limit is proportional to $M_{H^\pm}^2-M_A^2$. Hence, at high $M_A$, a partial cancellation between these diagrams is expected for nearly degenerate $M_{H^\pm}$ and $M_A$. Similarly, for $AA\ra ZZ$, a cancellation is possible when the masses $M_{H}$ and $M_A$ are close by. For $M_A \gtrsim 500$~GeV, keeping the mass differences of $M_{H^\pm}$ and $M_{H}$ with $M_A$ within $8$~GeV, such  cancellations help reproduce the correct $\Omega h^2$. It is nevertheless worth mentioning that such nearly degenerate masses will lead to coannihilation of  these $Z_2$ odd ID scalars~\cite{griest} to SM particles.
Despite such near-degeneracy, both $H$ and $H^+$, being charged under the same $Z_2$ as $A$, decay promptly to the LOP $A$, so that they do not become relics. {\tt FeynRules}~\cite{Alloul:2013bka} along with {\tt micrOMEGAs}~\cite{Belanger:2010gh, Belanger:2013oya} used to compute the relic density of $A$. 

In Fig.~\ref{fig:relicvsmassIn}, the relic density against the dark matter mass have been shown. For Fig.~\ref{fig:relicvsmassIn}(a), $\Delta M_{H^\pm}=\Delta M_{H}=50$ GeV have been chosen, so the relic density is mainly dominated by the self-annihilation of the dark matter candidate. For three different values of Higgs portal coupling, $\lambda_S=0.002,~0.005,~0.008$, the relic density turns out in the right ballpark for the dark matter mass $65-70$ GeV. The dominant annihilation channels are, $AA\ra b \bar{b},W^{\pm}W^{\mp*}$. Fig.~\ref{fig:relicvsmassIn}(b), the relic density is in the right ballpark with dark matter mass around 600 GeV. In this case both the co-annihilation and annihilation of the dark matter play important role. In this region inert particles annihilate mainly to $W^{\pm}W^{\mp},ZZ,hh$. The blue band corresponds to the constraints coming from the WMAP and Planck data. The region which is allowed from the relic density is also allowed from the direct search of the dark matter.

DM direct detection experiments involve the $h$-mediated $t$-channel process $AN\ra AN$ with a cross-section proportional to $\lambda_S^2/M_A^2$ in the limit $M_A\gg m_N$: 
%%%%%%%%%%%%%%%%%
\begp
\allowdisplaybreaks \beq
 \sigma_{A,N} = \frac{m_r^2}{\pi} f_N^2 m_N^2\left(\frac{\lambda_S}{M_{A} M_h^2}\right)^2 \label{directcs}
\eeq
\eegp
%%%%%%%%%%%%%%%%%%%%
where $f_N\approx0.3$ is the form factor of the nucleus. $m_r$ represents the reduced mass of the nucleus and the scattered dark matter particle. 

Thus, $\lambda_S$ is constrained from non observation of DM signals at XENON\,100~\cite{Aprile:2011hi,Aprile:2012nq} and LUX~\cite{Akerib:2013tjd}. For $M_{A}= 70$~GeV, the ensuing bound from LUX~\cite{Akerib:2013tjd,dmtools} data at 1$\sigma$ is $|\lambda_S|< 0.007$.  

The constraint on $\lambda_S$ from DM direct detection experiments gets diluted with $M_A$ [see eqn.~\ref{directcs}]. Hence, for low DM mass, direct detection bounds are more effective. At high mass, the relic density constraints are likely to supersede these bounds. For example, for $M_{DM}= 573$~GeV, the upper limit on $|\lambda_S|$ is 0.138 from LUX. However, to satisfy the relic density constraints from the combined data of WMAP and Planck within 3$\sigma$, $\lambda_S$ can be as large as $0.07$ only.

Within the framework of the ID model, it is possible to explain the observations in various indirect DM detection experiments~\cite{Arhrib:2013ela, Modak:2015uda} for some regions of the parameter space.
In this work, such details have not included as such estimations involve proper understanding of the astrophysical backgrounds and an assumption of the DM halo profile which contain some arbitrariness. For a review of constraints on the ID model from astrophysical considerations see, for example, Ref.~\cite{Gustafsson:2010zz}.

\vskip 20pt
\noindent{\bf\underline {Sign of $\lambda_3$}}\\

Whether $\lambda_3$ can be taken as positive or negative depends on the following:
\begin{itemize}

\item
If the ID model is not the answer to the DM puzzle, so that both relic density and direct detection constraints can be evaded, no restriction exists on the possible sign of $\lambda_3(M_Z)$. Otherwise, the following two cases need be considered:
\begin{itemize}
\item
A negative $\lambda_3(M_Z)$ implies 
%%%%%%%%%%%%%%%%%
\beq
\lambda_S(M_Z) < -\frac{1}{v^2} (M_{H^\pm}^2-M_A^2) \nn\, .
\eeq
%%%%%%%%%%%%%%%%%%%%
As $A$ is considered as the DM candidate, so that $M_A<M_{H^\pm}$, $\lambda_S(M_Z)$ is always negative when $\lambda_3(M_Z)<0$. 
For low DM mass, the splitting  $(M_{H^\pm}-M_A)\gtrsim 10$~GeV, as otherwise DM coannihilation processes cause an inappreciable  depletion in $\Omega h^2$. For $M_A=70$~GeV, this implies a lower bound $\lambda_S(M_Z)\lesssim -0.025$, which violates the DM direct detection bound $|\lambda_S|< 0.007$. Hence, for low DM mass, a negative $\lambda_3(M_Z)$  is not feasible.
\item
For high mass DM, the right relic density can be obtained when the splitting  $(M_{H^\pm}-M_A)\sim$ a few GeV or less. The above logic then implies that a negative $\lambda_3$ does not put any severe restriction on $\lambda_S$ to contradict DM direct detection bounds as earlier. Hence, for a high DM mass, $\lambda_3(M_Z)$ can assume both the signs. Moreover, due to propagator suppression for large $M_{H^\pm}$ in the $h\gamma\gamma$ vertex, the ID contribution to $\mu_{\gamma\gamma}$ is negligibly small and hence, the sign of $\lambda_3(M_Z)$ is not constrained by measurements on $\mu_{\gamma\gamma}$ as well. 
\end{itemize}
\item
If at any scale, $\lambda_3$ is negative while $\lambda_1>0$, then the bound~(\ref{stabilitybound}) must be respected. 
\item
If at some scale, $\lambda_1<0$, then a negative $\lambda_3$ makes the potential unbounded from below, as mentioned in the following section. This means one can start with a negative $\lambda_3(M_Z)$, but with RG evolution when $\lambda_1$ turns negative, $\lambda_3$ evaluated at that scale must be positive. Such parameter space does exist.
Here, a significant deviation has been found of this analysis from earlier analyses which did not allow a negative $\lambda_1$. For example, in Ref.~\cite{Goudelis:2013uca} a negative $\lambda_3(M_Z)$ was not allowed from stability of the Higgs potential if the theory has to be valid up to $10^{16}$~GeV together with relic density considerations. 
\end{itemize}
%%%%%%%%%%%%%%%%%
\subsection{Tunneling Probability and Metastability in IDM}
\label{sec:metastability}
 %%%%tunneling probability
 \begin{figure}[h!]
 \begin{center}
\subfigure[]{
 \includegraphics[width=2.7in,height=2.7in, angle=0]{./Plots/Inert_Tunnelingplots573}}
 \hskip 15pt
 \subfigure[]{
 \includegraphics[width=2.7in,height=2.7in, angle=0]{./Plots/tunnelinglamSplots}}
 \caption{\label{fig:TunIDM} \textit{ (a) Tunneling probability ${\cal P}_0$ dependence on  $M_t$. The left band (between dashed lines) corresponds to {\rm SM}. The right one (between dotted lines) is for $ID$ model for DM mass $M_A=573$~GeV.  Constraints from WMAP and Planck measured relic density, as well as XENON\,100 and LUX DM direct detection null results are respected for these specific choice of parameters. Light-green band stands for $M_t$ at $\pm 1\sigma$. (b) ${\cal P}_0$ is plotted against Higgs dark matter coupling $\lambda_S(M_Z)$ for different values of $\lambda_2(M_Z)$.}}
 \end{center}
 \end{figure}
%%%%tunneling probability

The presence of the inert doublet induces additional contributions to $\beta_{\lambda_1}$ (see eqn.~\ref{betal_1}).  As a result, which is generic for all scalars, $\lambda_1$ receives a positive contribution compared to the SM, which pushes a metastable vacuum towards stability, implying a lower ${\cal P}_0$ (see eqn.~\ref{prob}).

Electroweak metastability in the ID model has been explored earlier in the literature, albeit in a different context~\cite{Barroso:2013awa,Barroso:2012mj,Barroso:2013kqa,Gil:2012ya}. If $H^+$ gets a VEV, there could exist another charge-violating minimum. If instead, $A$ receives a VEV, another $CP$-violating minimum could pop up. But these vacua always lie higher than the usual EW vacuum. If $Z_2$ is broken by introducing additional soft terms in the Lagrangian, then the new $Z_2$-violating minimum can be lower than the usual $Z_2$-preserving EW minimum. As in this work, $Z_2$ is an exact symmetry of the scalar potential, so such cases need not be considered. However, as mentioned earlier, if at some scale before $\mpl$, the sign of $\lambda_1$ becomes negative, there might exist a deeper minimum which is charge-, $CP$- and $Z_2$-preserving and lying in the SM Higgs $h$ direction. 

The EW vacuum is metastable or unstable, depends on the minimum value of $\lambda_1$ before $\mpl$, which can be understood as follows. For EW vacuum metastability, the decay lifetime should be greater than the lifetime of the Universe, implying ${\cal P}_0 < 1$ (eqn.~\ref{lamminSM}).
Hence the vacuum stability constraints on the ID model can now be reframed, when $\lambda_{\rm 1, eff}$ runs into negative values, implying metastability of the EW vacuum.
It is reminded to the reader that in the ID model, instability of the EW vacuum cannot be realized as addition of the scalars only improves the stability of the vacuum. 
\begin{itemize}
\item
If $0>\lambda_{\rm 1, eff}(\Lambda_B)>\lambda_{\rm 1,min}(\Lambda_B)$, then the vacuum is metastable. 
\item
If $\lambda_{\rm 1, eff}(\Lambda_B)<\lambda_{\rm 1,min}(\Lambda_B)$, then the vacuum is unstable. 
\item
If $\lambda_2<0$, then the potential is unbounded from below along the $H, A$ and $H^\pm$ direction. 
\item
If $\lambda_3(\Lambda_{\rm I})<0$, the potential is unbounded from below along a direction in between $H^\pm$ and $h$.
\item
If $\lambda_L(\Lambda_{\rm I})<0$, the potential is unbounded from below along a direction in between $H$ and $h$.
\item
If $\lambda_S(\Lambda_{\rm I})<0$, the potential is unbounded from below along a direction in between $A$ and $h$.
\end{itemize}
In the above, $\Lambda_{\rm I}$ represents any energy scale for which $\lambda_{\rm 1, eff}$ is negative and the conditions for unboundedness of the potential follow from eqn.~\ref{Scalarpot2}.
At this point note the significant deviations are being made in the allowed parameter space compared to the usual vacuum stability conditions:  According to eqn.~\ref{stabilitybound}, $\lambda_{3,L,S}$ can take slightly negative values.
But at a scale where $\lambda_{\rm 1,eff}$ is negative, with the new conditions $\lambda_{3,L,S}$ have to be positive.

The tunneling probability ${\cal P}_0$ is computed by putting the minimum value of $\lambda_{\rm 1, eff}$ in eqn.~\ref{Action} to minimize $S(\Lambda_B)$.
In Fig.~\ref{fig:TunIDM}$\rm{ \left(a\right)}$, ${\cal P}_0$ has been plotted as a function of $M_t$.
The right band corresponds to the tunneling probability for our benchmark point as in Table~\ref{table1IDM}. For comparison, ${\cal P}_0$ has been plotted for SM as the left band in Fig.~\ref{fig:TunIDM}$\rm{(a)}$. 1$\sigma$ error bands in $\alpha_s$ and $M_h$ are also shown. As expected, for a given $M_t$, the presence of ID lowers tunneling probability. This is also reflected in Fig.~\ref{fig:TunIDM}$\rm {\left(b\right)}$, where ${\cal P}_0$ has been plotted as a function of  $\lambda_S(M_Z)$ for different choices of $\lambda_2(M_Z)$, assuming  $M_h=125.7$~GeV, $M_t=173.1$~GeV, and $\alpha_s=0.1184$. Here DM mass $M_A$ is also varied with $\lambda_S$ to get  $\Omega h^2=0.1198$. For a given $\lambda_S(M_Z)$, the higher the value of $\lambda_2(M_Z)$, the smaller ${\cal P}_0$ gets, leading to a more stable EW vacuum.

\subsection{Phase diagrams in IDM}  
\label{sec:phasediag}
The stability of EW vacuum depends on the value of parameters at low scale, chosen to be $M_Z$. In order to show the explicit dependence of EW stability on various parameters, it is customary to present phase diagrams in various parameter spaces.
%%%%ContourSTU
 \begin{figure}[h!]
 \begin{center}
% \subfigure[]{
 \includegraphics[width=2.7in,height=2.7in, angle=0]{./Plots/MHvsMDMcontourplot}
% \hskip 15pt
% \subfigure[]{
% \includegraphics[width=2.7in,height=2.7in, angle=0]{metastableinertSTUplot70unitary}}
 \caption{\label{fig:STU1} \textit{Constraints in $M_{H}-M_{A}$ plane in {\rm IDM}. The cross-hatched region  is excluded from LEP~{\rm \cite{Lundstrom:2008ai}}.  Choosing $M_{H^\pm}=120$~GeV and $\lambda_S(M_Z)=0.001$, relic density constraint is satisfied at 3$\sigma$ on the blue band. The green (yellow) region corresponds to EW vacuum stability (metastability). The solid brown line correspond to $M_H=M_A$. The gray area on the left to it is of no interest to us as $M_H>M_A$ has been chosen. The dashed brown line shows the LEP\,I limit. On the brown region, unitarity constraints are violated before $\mpl$. } }
 \end{center}
 \end{figure} 
%%%%ContourSTU
In Fig.~\ref{fig:STU1} the LEP constraints has been shown in the $M_{H}- M_A$ plane as in Ref.~\cite{Lundstrom:2008ai}.
Identifying regions of EW stability and metastability, the plot has been updated here.
As a scenario is being considered where the ID model is valid till $\mpl$, there are further limits from unitarity.
The relic density constraint imposed by WMAP and Planck combined data is represented by the thin blue band. The choice of $\lambda_2(M_Z)$ does not have any impact on relic density calculations, but affects EW stability as expected. In this plot, for higher values of $\lambda_2(M_Z)$, the region corresponding to EW metastability will be smaller. The chosen parameters  satisfy the LUX direct detection bound. 

%%%%ContourSTU
 \begin{figure}[h!]
 \begin{center}
% \subfigure[]{
% \includegraphics[width=2.7in,height=2.7in, angle=0]{MHvsMDMcontourplot}}
% \hskip 15pt
% \subfigure[]{
 \includegraphics[width=2.7in,height=2.7in, angle=0]{./Plots/metastableinertSTUplot70unitary}
 \caption{\label{fig:STU2} \textit{Phase diagram in $\Delta M_{H}-\Delta M_{H^\pm}$ plane for $M_A=70$~GeV in {\rm IDM}. The green and yellow regions correspond to EW vacuum stability and metastability respectively. The cross-hatched band is excluded from LEP. The brown region suffers from unitarity violation before $\mpl$. The blue band reflects relic density constraint at 3$\sigma$.
  } }
 \end{center}
 \end{figure} 
%%%%ContourSTU

As small splitting among $M_A$, $M_H$, and $M_{H^\pm}$ leads to some cancellations among diagrams contributing to DM annihilation, $\Delta M_{H^\pm}$ and $\Delta M_{H}$ are often used as free parameters in the ID model. In Fig.~\ref{fig:STU2}, constraints on this parameter space for $M_A=70$~GeV has been presented. As before, the brown region corresponds to unitarity violation before $\mpl$. For small $\Delta M_{H^\pm}$ and $\Delta M_{H}$, $\lambda_{3,4,5}$ are required to be small, which leads to little deviation from SM metastability. The metastable region is shown by the yellow patch, which shrinks for larger $\lambda_2$. The blue band reflects the relic density constraint for $\lambda_S(M_Z)=0.001$. For such small $\lambda_S(M_Z)$, the $h$-mediated $s$-channel diagram in $AA\ra WW$ or $AA\ra ZZ$ contributes very little. $H^+$- or $H$-mediated $t$- and $u$-channel diagrams are also less important than the quartic vertex driven diagram due to propagator suppression. This explains the ``L'' shape of the blue band. For higher values of $\lambda_S(M_Z)$, the shape of the band changes and ultimately leads to a closed contour. It appears that due to LEP constraints, EW vacuum metastability is almost ruled out. Although the LEP constraint permits $\Delta M_H<8$~GeV, allowing a narrow strip towards the left, the relic density constraints cannot be satisfied on this strip as it leads to an increased rate of DM coannihilation processes, leading to a dip in $\Omega h^2$. But as it will be seen later, if $M_t$ and $\alpha_s$ are allowed to deviate from their respective central values, for some region in this parameter space, it is possible to realize a metastable EW vacuum.    

%%%%MDMvsLamSphase
 \begin{figure}[h!]
 \begin{center}
 \subfigure[]{
 \includegraphics[width=2.7in,height=2.7in, angle=0]{./Plots/LamsMDMcontourplot}}
 \hskip 15pt
 \subfigure[]{
 \includegraphics[width=2.7in,height=2.7in, angle=0]{./Plots/LamsMDMcontourplothigh}}
 \caption{\label{fig:MDM_LamS} \textit{Phase diagram in $\lambda_S(M_Z)-M_A$ plane for $\lambda_2(M_Z)=0.1$ in {\rm IDM}. Panel (a) stands for `low' DM mass. The blue band  corresponds the 3$\sigma$ variation in $\Omega h^2$ when $\Delta M_{H^\pm}=40$~GeV and $\Delta M_H=40$~GeV. LEP direct search constraints are represented by the cross-hatched band at the bottom. Entire green region imply EW vacuum stability. Panel (b) stands for `high' DM masses.  The relic density band (blue) now correspond to  $\Delta M_{H^\pm}=1$~GeV and $\Delta M_H=2$~GeV. The corresponding stable and metastable phases for EW vacuum are represented by green and yellow patches respectively.   The relic density band (red) corresponds to  $\Delta M_{H^\pm}=5$~GeV and $\Delta M_H=2$~GeV. For this, the boundary separating the EW phases is denoted by the red dashed line.} }
 \end{center}
 \end{figure}
%%%%MDMvsLamSphase

To delineate the role of $M_H$ in EW vacuum stability, in Figs.~\ref{fig:STU1} and~\ref{fig:STU2}, $\lambda_2(M_Z)$ is chosen to be small. To demonstrate the effect of $\lambda_S$, phase diagrams will be presented in Fig.~\ref{fig:MDM_LamS} in the $\lambda_S(M_Z) - M_A$ plane. Panel (a) deals with low DM masses. For $\Delta M_{H^\pm}=40$~GeV and $\Delta M_H=40$~GeV, part of the allowed relic density band (blue) is allowed from LEP constraints (cross-hatched band). The entire parameter space corresponds to EW vacuum stability. Choosing small  $\Delta M_{H^\pm}$ and $\Delta M_H$, which imply small values of $\lambda_{3,4,5}$, can lead to metastability. But those regions are excluded by LEP. Again, metastability can creep in if $M_t$ and $\alpha_s$ are allowed to deviate from  their central values. 

In Fig.~\ref{fig:MDM_LamS}(b), the same parameter space has been studied for high DM masses. As mentioned before, to obtain the correct relic density, smaller mass splitting among various ID scalars needs to be chosen. For $\Delta M_{H^\pm}=1$~GeV and $\Delta M_H=2$~GeV, the 3$\sigma$ relic density constraint is shown as the blue band. The blue dashed line demarcates the boundary between stable (green) and metastable (yellow) phases of EW vacuum. The choice of small values of $\Delta M_{H^\pm}$ and $\Delta M_H$, in turn, leads to a large region pertaining to EW metastability. 

To illustrate the sensitivity to the mass splitting, in Fig.~\ref{fig:MDM_LamS}(b), another relic density band (red) has been presented for $\Delta M_{H^\pm}=5$~GeV and $\Delta M_H=2$~GeV. The corresponding boundary between the phases is denoted by the red dashed line. The region on the right implies EW stability (the green and yellow regions do not apply to this case). As for high DM masses, EW metastability can be attained for a sizable amount of the parameter space; $\lambda_2(M_Z)$ need not be chosen to be very small to maximize the metastable region for the sake of demonstration. 

The fact that for SM the EW vacuum stability is ruled out at $\sim 3\sigma$, is demonstrated by a phase space diagram in the $M_t-M_h$ plane~\cite{Degrassi:2012ry, Buttazzo:2013uya}. In Ref.~\cite{Khan:2014kba}, similar diagrams were presented for a singlet scalar extended SM. To demonstrate the impact of ID scalars to uplift the EW vacuum metastability, phase diagrams have been presented in the $M_t-M_h$ plane for two sets of benchmark points in Fig.~\ref{fig:Mt_MhIDM}. Panel (a) is drawn for $M_A = 70$~GeV, $\Delta M_{H^\pm}=11.8$~GeV, $\Delta M_H=45$~GeV, $\lambda_S(M_Z)=0.001$, and $\lambda_2 (M_Z) = 0.1$. For panel (b) the set of parameters in Table~\ref{table1IDM} is being used.
%%%%mtmhphase
 \begin{figure}[h!]
 \begin{center}
 \subfigure[]{
 \includegraphics[width=2.7in,height=2.7in, angle=0]{./Plots/MhMtcpoddplot70}}
 \hskip 15pt
 \subfigure[]{
 \includegraphics[width=2.7in,height=2.7in, angle=0]{./Plots/MhMtcpoddplot573}}
 \caption{\label{fig:Mt_MhIDM} \textit{Phase diagrams in $M_h - M_t$ plane in {\rm IDM}. Panels (a) and (b) stand for `low' and `high' DM masses respectively. Regions of 
absolute stability~(green), metastability~(yellow), instability~(red) of the EW vacuum are also marked. The gray zones represent error ellipses at  $1$, $2$ and  $3\sigma$. The three boundary lines (dotted, solid and dotted red) correspond to $\alpha_s(M_Z)=0.1184 \pm 0.0007$. Details of benchmark points are available in the text. } }
 \end{center}
 \end{figure}
%%%%mtmhphase 
Both sets of parameters are chosen so that they respect the WMAP and Planck combined results on DM relic density and the direct detection bounds from XENON\,100 and LUX. As in Ref.~\cite{Khan:2014kba}, the line demarcating the boundary between stable and metastable phases of EW vacuum is obtained by demanding that the two vacua be at the same depth, implying $\lambda_1(\Lambda_B)=\beta_{\lambda_1}(\Lambda_B)=0$. The line separating the metastable phase from the unstable one is drawn using the conditions $\beta_{\lambda_1}(\Lambda_B)=0$ and $\lambda_1(\Lambda_B)=\lambda_{1, \rm min}(\Lambda_B)$, as in eqn.~\ref{lamminSM}. The variations due to uncertainty in the measurement of $\alpha_s$ are marked as dotted red lines. In each panel, the dot representing central values for $M_h$ and $M_t$ is encircled by 1$\sigma$, 2$\sigma$, and 3$\sigma$ ellipses representing errors in their measurements.  According to Fig.~\ref{fig:Mt_MhIDM}(a), EW vacuum stability is allowed at 1.5$\sigma$, whereas in Fig.~\ref{fig:Mt_MhIDM}(b), it is excluded at 2.1$\sigma$, indicated by blue-dashed ellipses.

%%%%Mt-alphaS phase diagram
  \begin{figure}[h!]
 \begin{center}
 \subfigure[]{
 \includegraphics[width=2.7in,height=2.7in, angle=0]{./Plots/AlphavsmtplotsCPodd70}}
 \hskip 15pt
 \subfigure[]{
 \includegraphics[width=2.7in,height=2.7in, angle=0]{./Plots/AlphavsmtplotsCPodd573}}
 \caption{\label{fig:Alpha_MtIDM} \textit{ Phase diagrams in $M_t-\alpha_s(M_Z)$ plane in {\rm IDM} for the same sets of benchmark points as in Fig.~\ref{fig:Mt_MhIDM}. Notations used are also the same as in Fig.~\ref{fig:Mt_MhIDM}. } }
 \end{center}
 \end{figure}
%%%%Mt-alphaS phase diagram 
As in the literature SM EW phase diagrams are also presented in the $\alpha_s(M_Z)-M_t$ plane~\cite{Bezrukov:2012sa, EliasMiro:2011aa}, the same is done in the ID model as well. In Fig.~\ref{fig:Alpha_MtIDM}, the same sets of benchmark parameters has been used as in Fig.~\ref{fig:Mt_MhIDM}. As a consistency check, one can note that the EW vacuum is allowed or ruled out at the same confidence levels.
%%%%confidence
 \begin{figure}[h!]
 \begin{center}{
 \includegraphics[width=2.7in,height=2.7in, angle=0]{./Plots/lamsconfdncplot44}}
 \caption{\label{fig:confidenceIDM} \textit{ Dependence of confidence level at which EW vacuum stability is excluded (one-sided) or allowed on $\lambda_S(M_Z)$ and $\lambda_2(M_Z)$ in {\rm IDM}. Regions of absolute stability (green) and metastability (yellow) of EW vacuum are shown for $\lambda_2(M_Z)=0.1$. The positive slope of the line corresponds to the stable EW vacuum and negative slope corresponds to the metastability.     
 } }
 \end{center}
 \end{figure}
%%%%confidence

To study the impact of nonzero ID couplings, however, it is instructive to study the change in the confidence level ($\sigma$) at which EW stability is modified with respect to these couplings. As in Ref.~\cite{Khan:2014kba}, In Fig.~\ref{fig:confidenceIDM} ~$\sigma$ has been plotted against $\lambda_S(M_Z)$ for different values of $\lambda_2(M_Z)$. $M_A$ is varied along with $\lambda_S(M_Z)$ to keep DM relic density fixed at $\Omega h^2=0.1198$ throughout the plot. Note that changing $\lambda_2(M_Z)$ does not alter $\Omega h^2$. The masses of other ID particles  are determined using $\Delta M_{H^\pm}=1$~GeV and $\Delta M_H=2$~GeV. The parameter space considered does not yield too large DM-nucleon cross-section, inconsistent with XENON\,100 and LUX DM direct detection null results. For a specific value of $\lambda_2(M_Z)=0.1$, with the increase of $\lambda_S(M_Z)$, the confidence level at which EW is metastable (yellow region) gets reduced and becomes zero at $\lambda_S(M_Z)\simeq 0.04$. After this, EW vacuum enters in the stable phase (green). With further increases in $\lambda_S(M_Z)$, the confidence level at which EW is stable keeps increasing.
Two other values in the same plot is used to illustrate the role of $\lambda_2(M_Z)$.
The value of $\lambda_S(M_Z)$ at which the EW vacuum enters in the stable phase increases with decreases in $\lambda_2(M_Z)$, as expected. The yellow and green marked regions are not applicable when $\lambda_2(M_Z)=0.05, 0.15$.   
\subsection{Veltman's conditions in IDM}
\label{sec:veltman}
%%%%%%%%%%%%%%%%%%%%%%%%%
As the validity of the ID model have been extended till $\mpl$, it is interesting to explore whether Veltman's condition (VC) can be satisfied in this model at any scale on or before $\mpl$. It has been shown in Section~\ref{VCsINSM}, if one imposes VC in the SM at $\mpl$, then the top mass measurement $M_t=173.1\pm 0.6$~GeV implies $M_h\approx 135\pm2.5$~GeV, which is excluded at more than 5$\sigma$.  

Veltman's condition implies that the quadratic divergences in the radiative corrections to the Higgs mass can be handled if the coefficient multiplying the divergence somehow vanishes~\cite{Veltman:1980mj, Hamada:2012bp}. VC includes the contributions from the infrared degrees of freedom of the theory and does not carry any special information about the ultraviolet divergences. In SM, it suggests the combination 
%%%%%%%%%%%%%%%%%
\begp
\allowdisplaybreaks \beq
6 \lambda_1+\frac{9}{4} g_2^2+\frac{3}{4} g_1^2 -12 y_t^2 = 0\nn\, .
\eeq
\eegp
%%%%%%%%%%%%%%%%%%%%
Due to the large negative contribution from the term containing the top Yukawa coupling, it is not possible to satisfy VC till $\mpl$ given the experimental measurements of $M_t$ and $M_h$ within the context of SM.

In the ID model, as more scalars are added a possibility opens up to satisfy VC, as their contributions can offset the large negative contribution from the top quark. 

The above VC for the SM associated with $m_{11}$ is promoted in the ID model to~\cite{Barbieri:2006dq, Chakraborty:2014oma}
%%%%%%%%%%%%%%%%%
\begp
\allowdisplaybreaks \beq
6 \lambda_1+ 2\lambda_3+\lambda_4+\frac{9}{4} g_2^2+\frac{3}{4} g_1^2 -12 y_t^2  = 0.
\eeq
\eegp
%%%%%%%%%%%%%%%%%%%%
If $2\lambda_3+\lambda_4$ is positive, then it has been checked with the RG improved coupling constants, and it is possible to satisfy the above VC at a scale before $\mpl$. 

However, in the ID model $m_{22}$ also receives quadratically divergent radiative corrections. The corresponding VC reads as
%%%%%%%%%%%%%%%%%
\begp
\allowdisplaybreaks \beq
6 \lambda_2+ 2\lambda_3+\lambda_4+\frac{9}{4} g_2^2+\frac{3}{4} g_1^2 = 0\, .
\eeq
\eegp
%%%%%%%%%%%%%%%%%%%%
Note that it lacks the Yukawa contribution as the unbroken $Z_2$ forbids fermionic interactions of the inert doublet $\Phi_2$. As $2\lambda_3+\lambda_4$ is already positive, this VC can be satisfied if $\lambda_2$ is negative. But a negative $\lambda_2$ renders the potential unbounded from below as evident from the earlier discussions. Note that amongst our RG improved coupling constants $\lambda_1$ can be driven to negative values at high scales. But this makes the required cancellations for VCs even worse. Hence, it is not possible to satisfy Veltman's conditions in a scenario where only the ID model reigns the entire energy regime up to the $\mpl$. 


\section{Triplet ($Y=0$) scalar extension of the SM}
\label{sec:ITM}
In this case, the SM is extended by an additional hyperchargeless ${ SU(2)_L}$ scalar triplet. This triplet is odd under a discrete $Z_2$ symmetry, whereas, the standard model fields are even. Also this symmetry prohibits the inert triplet to acquire a vacuum expectation value.

The tree-level scalar potential of eqn.~\ref{ScalarpotHTM} with  additional $Z_2$-symmetry, can be written\footnote{Here $T$ is denoted as the scalar triplet, which is equivalent to $\widetilde{\Phi}$ of eqn.~\ref{TripPhiY0} and the $\lambda_i$'s are equivalent to $\widetilde{\lambda}_i$ of the eqn.~\ref{ScalarpotHTM}.} as, 
%%%%%%%%%%%%%%%%%%
\begp
\allowdisplaybreaks \bea
V_0(\Phi,T) &=& \mu_1^2 |\Phi|^2 + \lambda_1 |\Phi|^4+ \frac{\mu_2^2}{2} ~tr|T|^2 + \frac{\lambda_2}{4} ~tr|T|^4+ \frac{\lambda_3}{2} |\Phi|^2 tr|T|^2   \, ,
\label{ScalarpotHTM1}
\eea
\eegp
%%%%%%%%%%%%%%%%%%%%
where the SM Higgs doublet $\Phi$ and the inert scalar triplet $T$ are given by,
%%%%%%%%%%%%%%%%%
%\renewcommand*{\arraystretch}{0}{
\begp
\allowdisplaybreaks \beq
	\Phi ~=~ \left( \begin{array}{c} G^+ \\ \frac{1}{\sqrt{2}}\left(v+h+i G^0\right) \end{array} \right),
	\qquad
	T ~=~ \left(
\begin{array}{cc}
   H/\sqrt{2}  &   -H^+ \\
     -H^- &  -H/\sqrt{2} 
\end{array}\right),
\eeq
\eegp
%%%%%%%%%%%%%%%%%%%%
$T$ contains a neutral scalar $H$ and a pair of charged scalar fields $H^\pm$. The $Z_2$ symmetry prohibits these particles to decay entirely to SM particles. The neutral particle $H$ can then serve as a DM candidate. 

After electroweak symmetry breaking the scalar potential can be written as,
%%%%%%%%%%%%%%%%%%
\begp
\allowdisplaybreaks \bea
V(h, H,H^\pm) &=&  \frac{1}{4} \left[ 2 \mu_1^2 (h+v)^2 + \lambda_1 (h+v)^4 +2 \mu_2^2 (H^2+2 H^+ H^-) \right. \nn \\
&& \left. + \lambda_2 (H^2 + 2 H^+ H^-)^2  + \lambda_3 (h+v)^2 (H^2+2 H^+ H^-) \right].\nn
\eea
\eegp
%%%%%%%%%%%%%%%%%%%%
Masses of these scalars are given by,
%%%%%%%%%%%%%%%%%%
\begp
\allowdisplaybreaks \begin{align}
	M_{h}^2 &= \mu_1^2 + 3 \lambda_1 v^2,\nn \\
	M_{H}^2 &= \mu_2^2 +  \frac{\lambda_3}{2} v^2, \nn \\
	M_{H^\pm}^2 &= \mu_2^2 + \frac{\lambda_3}{2}  v^2  \,\nn .
	\label{MassTrip}
\end{align}
\eegp
%%%%%%%%%%%%%%%%%%
At the tree level both the neutral and charged particle masses are the same. If we include one-loop radiative correction then the charged particles become slightly heavier~\cite{Cirelli:2009uv,Cirelli:2005uq} than neutral ones.
%%%%%%%%%%%%%%%%%
\begp
\allowdisplaybreaks \beq
\Delta M=(M_{H^\pm}-M_{H})_{1\text{-}loop}=\frac{\alpha M_{H}}{4\pi s_W^2}\Big[f(\frac{M_W}{M_{H}}) -c_W^2 f(\frac{M_Z}{M_{H}})\Big]\nn
\label{massdifftrip}
\eeq
\eegp
%%%%%%%%%%%%%%%%%%%%
where,
%%%%%%%%%%%%%%%%%
\begp
\allowdisplaybreaks \beq
f(x)=-\frac{x}{4}\Big[ 2 x^3 ~ {\rm log}(x)+(x^2-4)^{\frac{3}{2}}~ {\rm log}\Big[ \frac{1}{2}(x^2-2-x\sqrt{x^2-4}) \Big]\Big].\nn
\eeq
\eegp
%%%%%%%%%%%%%%%%%%%%
One-loop effective Higgs potential in $\MS$ scheme in the Landau gauge is given by   
%%%%%%%%%%%%%%%%%
\begp
\allowdisplaybreaks \beq
V_1^{{\rm SM}+{\rm IT}}(h)= V_1^{\rm SM}(h) + V_1^{\rm IT}(h)
\eeq
\eegp
%%%%%%%%%%%%%%%%%%%%
$V_1^{\rm SM}(h)$ can be found in eqn.~\ref{V1loop}. The additional contribution to the one-loop effective potential due to the inert triplet is given by~\cite{Forshaw:2003kh},
%%%%%%%%%%%%%%%%%
\begp
\allowdisplaybreaks \beq
V_1^{\rm IT}(h)= \sum_{j=H,H^+,H^-} \frac{1}{64 \pi^2} M_j^4(h) \left[ \ln\left(\frac{M_j^2(h)}{\mu^2(t)} \right)- \frac{3}{2} \right] 
\eeq
\eegp
%%%%%%%%%%%%%%%%%%%%
where, 
%%%%%%%%%%%%%%%%%
\begp
\allowdisplaybreaks \beq
M_j^2(h)=\frac{1}{2} \,\lambda_{j}(t) \, h^2(t)+\mu_2^2(t) 
\eeq
\eegp
%%%%%%%%%%%%%%%%%%%%
with $\lambda_{H,H^\pm}(t)= \lambda_{3}(t)$.
In the present work, in the Higgs effective potential, SM contributions are taken at two-loop level and the IT scalar contributions are considered at one-loop only. 

Similarly for large field value $h\gg v$, the Higgs effective potential can be approximated as
%%%%%%%%%%%%%%%%%
\begp
\allowdisplaybreaks \beq
V_{\rm eff}^{{\rm SM}+{\rm IT}}(h) \simeq \lambda_{\rm 1,eff}(h) \frac{h^4}{4}\, ,
\label{efflamIT}
\eeq
\eegp
%%%%%%%%%%%%%%%%%%%%
with
%%%%%%%%%%%%%%%%%
\begp
\allowdisplaybreaks \beq
\lambda_{\rm 1,eff}(h) = \lambda_{\rm 1,eff}^{\rm SM}(h) +\lambda_{\rm 1,eff}^{\rm IT}(h)\, ,
\label{lameffIT}
\eeq
\eegp
%%%%%%%%%%%%%%%%%%%%
where $\lambda_{\rm eff}^{\rm SM}(\phi)$ same as in eqn.~\ref{eq:effqurtic} and,
%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%
\begp
\allowdisplaybreaks \bea
 \lambda_{\rm 1,eff}^{\rm IT}(h)&=& e^{4\Gamma(h)} \left[\frac{3 \lambda_3^2}{256 \pi^2}  \left(\ln\left(\frac{\lambda_3}{2}\right)-\frac{3}{2}\right ) \right]\, . \label{efflamtriplet}
\eea
\eegp
%%%%%%%%%%%%%%%%%%%%
%%%%RGE RUNNING
 \begin{figure}[h!]
 \begin{center}
 % \subfigure[]{
 \includegraphics[width=2.7in,height=2.7in, angle=0]{./triplet/1couplingvsenergy_Triplet}
 \caption{\label{fig:SMInert} \textit{{\rm ITM} RG evolution of the couplings $\lambda_1, \lambda_2, \lambda_3$ for the set of parameters in Table~\ref{table1IT}. } }
 \end{center}
 \end{figure}
%%%%RGE RUNNING
%%%%%%%%%%%%%%%%%
%%%%%%%%%
%\renewcommand*{\arraystretch}{15}{
\setlength\tablinesep{2pt}
\begin{table}[h!]
\begin{center}
    \begin{tabular}{| c | c | c | c | c | c | c | c |}
    \hline
      & $\lambda_1$ & $\lambda_2$ &  $\lambda_3$\\
\hline
   ~$M_{t}$  ~&~ 0.127054 ~&~ 0.10 ~&~ 0.10~\\
            \hline
   $\mpl$ & $-$0.00339962 & 0.267706 & 0.206306\\
              \hline
    \end{tabular}
    \caption{A set of values of all ITM coupling constants at  $M_t$ and $\mpl$ for $M_{DM}=1897$ GeV.}
    \label{table1IT}
\end{center}
\end{table}
%%%%%%%%%%%%%%%%%
To compute the RG evolution of all the couplings in these model, we first calculate all couplings with threshold corrections at $M_t$ and using the RG-eqns.~\ref{betal_HTM}$-$\ref{betal_3HTM}, one can obtain the couplings $\lambda_{1,2,3}$ at $\mpl$.
For a specific set of values of $\lambda_i$ at $M_t=173.1$~GeV, their values at $\mpl = 1.2 \times 10^{19}$~GeV for $M_h=125.7$~GeV and $\alpha_s\left(M_Z\right)=0.1184$ have been provided in Table~\ref{table1IT}. In Fig.~\ref{fig:SMInert} we explicitly show running of the scalar couplings $(\lambda_i)$ for this set of parameters. It has been found that for the specific choice of parameters, $\lambda_1$ assumes a small negative value leading to a metastable EW vacuum as discussed in the previous sections.
%%%%%%%%%%%%%%%%%%%%
\subsection{Constraints on ITM}
%%%%%%%%%%%%%%%%%%%%%%
The absolute stability of the EW vacuum of the scalar potential (eqn.~\ref{ScalarpotHTM1}), unitarity of scattering matrix, perturbativity and the EW precision measurements puts a stringent bound on the ITM parameter space which had been shown in Chapter~\ref{chap:EWSBextended}.

Constrains from LHC diphoton signal strength and dark matter will be discussed in the following subsections.
%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Bounds from LHC diphoton signal strength}
The Higgs to diphoton signal strength $\mu_{\gamma\gamma}$ can be defined similar to eqn.~\ref{mugagalow}. If the IT particles have masses greater than $M_h/2$, i.e., $\Gamma\left(h\rightarrow \rm IT,IT\right)=0$ then,
%%%%%%%%%%%%%%%%%
\begp
\allowdisplaybreaks \beq 
 \mu_{\gamma\gamma}= \frac{\Gamma(h\rightarrow \gamma\gamma)_{\rm IT}}{\Gamma(h\rightarrow \gamma\gamma)_{\rm SM}}\, .
 \label{mugagahighIT}
\eeq
\eegp
%%%%%%%%%%%%%%%%%%%%
In ITM, the additional contributions to $\mu_{\gamma\gamma}$ at one-loop due to the $H^\pm$ can be found in eqn.~\ref{hgaga}, where $\mu_{hH^+H^-}= \lambda_3 v$ stands for the coupling constant of $hH^+H^-$ vertex.
 One can see that a positive $\lambda_3$ leads to a destructive interference between SM and IT contributions in eqn.~\ref{hgaga} and {\it vice versa}. Hence, for IT particles heavier than $M_h/2$, $\mu_{\gamma\gamma}<1$ ($\mu_{\gamma\gamma}>1$) when $\lambda_3$ is positive (negative).
One can see from the eqn.~\ref{hgaga}, the contribution to the Higgs diphoton channel is proportional to $\frac{\lambda_3}{M_{H^\pm}^2}$.
It has been seen, if the charged scalar mass is greater than $300$ GeV then the contributions of inert triplet model to the diphoton signal is negligible.
%%%%%%%%%%%%%%%%%%%%
\subsubsection{Constraints from dark matter relic density}
%%%%%%%%%%%%%%%%%
\begin{figure}[h!]
\begin{center}
{
\includegraphics[width=2.7in,height=2.7in, angle=0]{./triplet/TripletRelivsMDM}}
\caption{ \textit{Dark matter relic density $\Omega h^2$ as a function of the dark matter mass $M_{DM}(\equiv M_H)$ for the portal coupling: $\lambda_3(M_Z)=0.10$ (red) in {\rm ITM}. The thin blue band corresponds the relic density, $\Omega h^2=0.1198 \pm 0.0026$ (3$\sigma$).}}
\label{fig:relictriplet}
\end{center}
\end{figure}
%%%%%%%%%%%%%%%%%%%%
In Fig.~\ref{fig:relictriplet}, we have plotted the relic density as a function of dark matter mass for ITM. Here in this plot, the Higgs portal coupling $\lambda_3(M_Z)=0.10$ has been used. The light red band is excluded from the Higgs invisible decay width data from the LHC. It has been seen that from eqn.~\ref{massdifftrip}, the mass difference between the neutral and charged particles is $\sim$150 MeV~\cite{Cirelli:2009uv,Cirelli:2005uq}. The co-annihilation cross-section of the dark matter $H$ with charged ($H^\pm$) particles are very large. It has been seen that for 500 GeV, the total cross-section is $\left\langle \sigma v \right\rangle \sim 10^{-25}$ ${\rm cm^3 s^{-1}}$ and so the relic density becomes $\sim 0.01$ which corresponds to under-abundance. For dark matter mass greater than $1.8$ TeV, one can get relic density of the dark matter in the right ballpark. 

%%%%%%%%%%%%%%%%%%%%%%
\subsection{Tunneling Probability and Metastability in ITM}\label{TUNHTM}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\label{sec:metastabilityIT}
 %%%%tunneling probability
 \begin{figure}[h!]
 \begin{center}
\subfigure[]{
 \includegraphics[width=2.7in,height=2.7in, angle=0]{./triplet/1Triplet_Tunnelingplots}}
 \hskip 15pt
 \subfigure[]{
 \includegraphics[width=2.7in,height=2.7in, angle=0]{./triplet/1tunnelinglamSplots1}}
 \caption{\label{fig:TunIT} \textit{ (a) Tunneling probability ${\cal P}_0$ dependence on  $M_t$. The left band (between dashed lines) corresponds to {\rm SM}. The right one (between dotted lines) is for $IT$ model for DM mass $M_H=1897$~GeV. Dark matter constraints are respected for these specific choices of parameters. Light-green band stands for $M_t$ at $\pm 1\sigma$. (b) ${\cal P}_0$ is plotted against Higgs dark matter coupling $\lambda_S(M_Z)$ for different values of $\lambda_2(M_Z)$.}}
 \end{center}
 \end{figure}
%%%%tunneling probability
The tunneling probability ${\cal P}_0$ (see eqn.~\ref{prob}) is computed by putting the minimum value of $\lambda_{1,\rm eff}$ of eqn.~\ref{lameffIT} in eqn.~\ref{Action}. In Fig.~\ref{fig:TunIT}$\left(a\right)$, we have plotted  ${\cal P}_0$ as a function of  $M_t$. The right band corresponds to the tunneling probability for our benchmark point as in Table~\ref{table1IT}. For comparison, we plot ${\cal P}_0$ for SM as the left band in Fig.~\ref{fig:TunIT}$(a)$. 1$\sigma$ error bands in $\alpha_s$ and $M_h$ are also shown. We plot ${\cal P}_0$ as a function of  $\lambda_3(M_Z)$ in Fig.~\ref{fig:TunIT}$\left(b\right)$ for different choices of $\lambda_2(M_Z)$, assuming  $M_h=125.7$~GeV, $M_t=173.1$~GeV and $\alpha_s=0.1184$. Here DM mass $M_{DM}$ is also varied with $\lambda_3$ to get  $\Omega h^2=0.1198$.

The modified vacuum stability conditions are, 
\begin{itemize}
\item
If $0>\lambda_1(\Lambda_B)>\lambda_{\rm 1,min}(\Lambda_B)$, then the vacuum is metastable. 
\item
If $\lambda_1(\Lambda_B)<\lambda_{\rm 1,min}(\Lambda_B)$, then the vacuum is unstable. 
\item
If $\lambda_2<0$, the potential is unbounded from below along the $H$ and $H^\pm$-direction. 
\item
If $\lambda_3(\Lambda_{\rm I})<0$, the potential is unbounded from below along a direction in between $H$ and $h$ also $H^\pm$ and $h$.
\end{itemize}
In the above, $\Lambda_{\rm I}$ represents any energy scale for which $\lambda_1$ is negative. 
%%%%%%%%%%%%
\subsection{Phase diagrams in ITM}
%%%%Mt-alphaS phase diagram 
%In Fig.~\ref{fig:Mt_MhScalar} and Fig.~\ref{fig:Mt_MhIDM}, similar diagrams were presented for a singlet and inert doublet extended scalar of SM.
%%%%%%%%%%%%%%%%
%%%%Mt-alphaS phase diagram
 \begin{figure}[h!]
 \begin{center}
 \subfigure[]{\includegraphics[width=2.7in,height=2.7in, angle=0]{./triplet/1MhMttripletplot}}
 \hskip 15pt
  \subfigure[]{
 \includegraphics[width=2.7in,height=2.7in, angle=0]{./triplet/1Alphavsmtplots}}
 \caption{\label{fig:Mt_MhIT} \textit{Phase diagrams in (a) $M_h - M_t$ plane and (b) $M_t-\alpha_s(M_Z)$ plane {\rm ITM}. Regions of 
absolute stability~(green), metastability~(yellow), instability~(red) of the EW vacuum are also marked. The gray zones represent error ellipses at $1$, $2$ and  $3\sigma$. The three boundary lines (dotted, solid and dotted red) correspond to $\alpha_s(M_Z)=0.1184 \pm 0.0007$.
} }
 \end{center}
 \end{figure} 
 %%%%%%%%%%%%%%%%%%
To explain the impact of inert triplet scalars to uplift the EW vacuum metastability, in Fig.~\ref{fig:Mt_MhIT} phase diagram in $M_t-M_h$ and $\alpha_s(M_Z)-M_t$ plane has been presented for the benchmark points $M_{DM}=1897$ GeV, $\lambda	_2(M_Z)=0.10$ and $\lambda_3(M_Z)=0.10$. For this points one can see from the phase diagram in Fig.~\ref{fig:Mt_MhIT} that the stability electroweak is excluded at 1.2$\sigma$ (one-sided).
%%%%%%%%%%%%%%%%%%%%%%%%%
 %%%%confidence
 \begin{figure}[h!]
 \begin{center}{
 \includegraphics[width=2.7in,height=2.7in, angle=0]{./triplet/1lam3confdncplot}}
 \caption{\label{fig:confidenceIT} \textit{Dependence of confidence level  at which EW vacuum stability is excluded (one-sided) or allowed on $\lambda_3(M_Z)$ and $\lambda_2(M_Z)$ in {\rm ITM}. Regions of absolute stability (green) and metastability (yellow) of EW vacuum are shown for $\lambda_2(M_Z)=0.1$.% The positive slope of the line corresponds to the stable EW vacuum and negative slope corresponds to the metastability.     
 } }
 \end{center}
 \end{figure}
%%%%confidence
%%%%%%%%%%%%%%%

The confidence level vs $\lambda_3(M_Z)$ diagram like Fig.~\ref{fig:kappaconfidence} of SM+$S$ and Fig.~\ref{fig:confidenceIDM} of IDM is presented in Fig.~\ref{fig:confidenceIT} for the inert triplet model.
If the ITM is valid up to the Planck scale, which may saturate the relic abundance of the dark matter of the Universe then this phase diagram becomes important to realize where the present EW vacuum is residing. Along the line (black, blue and red) in the Fig.~\ref{fig:confidenceIT} the dark matter mass change in such a way that the relic density $\Omega h^2 = 0.1198$ remains same.
One can see that with the increase of $\lambda_{2,3}(M_Z)$, the EW vacuum approaches the stability. In this model, the electroweak vacuum becomes absolutely stable after $\lambda_3(M_Z)= 0.154$ for $\lambda_2(M_Z)\approx 0.10$ (see blue line in the Fig.~\ref{fig:confidenceIT}).
This phase diagram has been presented for central values of $M_h$, $M_t$ and $\alpha_s(M_Z)$. However, if we increase the top mass or decrease the Higgs mass or decrease $\alpha_s(M_Z)$ within experimental uncertainties then 
the size of the region corresponding to the metastability of the EW vacuum increases.
With a maximum top mass $M_t=174.9$ GeV and a minimum $M_h=124.8$ GeV and a minimum $\alpha_s(M_Z)=0.1163$, allowed at 3$\sigma$, the EW vacuum the Higgs potential becomes absolutely stable for the dark matter mass more than 1912 GeV with $\lambda_{3}(M_Z)$ greater than $0.31$ for fixed $\lambda_2(M_Z)=0.1$.
%%%%%%%%%%%%%%%%%%%%

In Fig.~\ref{fig:Rgammagamma}, we have shown the valid parameter spaces in $\lambda_3(M_Z)-M_H$ plane for central value of $M_t$, $M_h$ and $\alpha(M_Z)$. Here the lower (red) region are excluded, as the scalar potential becomes unbounded from below along the direction in between $H^\pm$ and $h$.
In this region the effective Higgs quartic coupling is negative and form a local minima along the Higgs $h$ direction near the Planck scale and at the same time $\lambda_3$ remains negative up to the Planck scale. It has been found that the parameter spaces with negative $\lambda_3(M_Z)$ is also allowed from the metastability.
In this case $\lambda_3$ becomes positive at the scale $\Lambda_{B}$ of global minimum and remains positive up to the Planck scale. The green region implies that the EW vacuum is absolutely stable. In the upper red region the unitary bounds are violated. In the plot, the right-side of the black dotted line are viable from $\mu_{\gamma\gamma}$ at 1$\sigma$.
%Note that in this plot, the relic density of the dark matter found is in under abundance.
%%%%%%%%%%%%%%%%
%%%%Gamma
 \begin{figure}[h!]
 \begin{center}
 % \subfigure[]{
 \includegraphics[width=3.0in,height=2.7in, angle=0]{./triplet/1Plotlam3vsMHch}
 \caption{\label{fig:Rgammagamma} \textit{Phase diagram in $\lambda_3(M_Z)-M_H$ plane in {ITM}. Right side of the black-dotted line is allowed from the signal strength ratio of $\mu_{\gamma\gamma}$ within 68$\%$ confidence level. and the left side is excluded at 1$\sigma$. In the metastable region, the Higgs portal coupling $\lambda_3(M_Z)$ is negative, however, beyond the scale $\Lambda_{B}$ it is greater than zero.} }
 \end{center}
 \end{figure}
%%%%Gamma

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Summary}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
According to the standard model of particle physics with the present measured values of the SM parameters, the electroweak vacuum is lying right in between stability and instability, as if it is ready to tunnel into a regime of absolute instability.
Nevertheless, the transition time required for this is safely beyond the present lifetime of the Universe. Still, the question is, what prompts such a near-criticality? In this chapter, we did not try to find an answer to this question. But we explored the validity of this question in the context of the different models containing extra scalar field(s) that also offers a solution to the dark matter puzzle.

Near-criticality is best explained with the help of phase
diagrams which were used in the Chapter~\ref{chap:MetaSM} for the SM.
A similar endeavor has been made in this chapter for various kinds of extended scalar sectors namely SM+$S$, inert doublet and inert triplet models.
The next-to-next-to-leading order corrections have been included in the SM calculations. The
effects due to the extra scalar(s) were incorporated up to two-loop.

In this chapter, various kinds of dark matter models have been chosen to illustrate changes in EW vacuum stability as apart from neutrino masses, the presence of dark matter in the Universe is the most striking signature of new physics beyond the standard model of particle physics.

In these models, for some specific choice of parameter space, the scalar field(s) can rescue the EW vacuum from metastability, making it absolutely stable, so that $\lambda$ never turns negative.
But as the DM direct detection experiments or collider searches are yet to confirm the exact nature of the DM candidate, the parameter space allowed by DM relic density constraints, dictated by the cosmic microwave background radiation experiments such as Planck or WMAP, have been considered.
It has been checked that in these considerations, the related DM-nucleon cross-sections are beyond the present sensitivity of direct-detection experiments such as XENON100 and LUX.

The addition of scalar multiplet does not help in realizing the asymptotic safety scenario of gravity. But it is possible to have two degenerate vacua at somewhat lower energy (shown for the SM+$S$ model), which depends on the parameter space under consideration.

In short, near-criticality of EW vacuum indicates the presence of new dynamics other than the SM at a very high energy.
In this chapter, new scalars physics have been introduced at EW scale to demonstrate the influence of such scalars in shaping the minimum (if any) of the potential lying close to $\mpl$.



















==> conclusions/conclusions.tex <==
\chapter{Summary and Conclusions}
\label{chap:Conclusions}
\linespread{0.1}
\pagestyle{headings}
\noindent\rule{15cm}{1.5pt} 

The Higgs signal strength data is consistent with the theoretical predictions of the SM with small uncertainties. The LHC is yet to find any convincing signal suggesting the existence of any new physics beyond the standard model of particle physics. There are several well-motivated possibilities for an enlarged scalar sector that go far beyond the minimalistic one doublet scenario of the standard model. Small uncertainty in Higgs signal data at LHC does allow physics beyond the SM. Other experimental evidences point towards the existence of dark matter, which so far could have escaped detection in colliders and DM direct detection experiments.

In this thesis, several extended scalar sectors of the SM have been discussed.
The SM has been extended with either a $SU(2)$ singlet or doublet or triplet with different hypercharges.
It has been considered that the extra scalar fields transform under same standard model gauge group.


This work has two aspects. In the first case, it has been considered that both the SM doublet and the extra scalar field are responsible for the electroweak symmetry breaking, i.e., both the neutral $CP$-even component of SM doublet and extra scalar fields are getting vacuum expectation values.
In other words, the minima of the combined scalar potential form on the plane containing the $CP$-even components. These components mix and form a Higgs-like particle and extra heavy scalar particles.
The different extended scalar sectors contain different kinds of scalar particles such as charged, or neutral $CP$-even and $CP$-odd scalar(s).
These scalars can couple to the vector bosons. In this point of view, various kinds of vector boson scattering processes have been calculated for the
three models such as $(i)$ type-II two Higgs doublet model, $(ii)$ Higgs triplet model with a hyperchargeless scalar triplet, and $(iii)$ Higgs triplet model with a
scalar triplet with hypercharge $Y = 2$.
The exact expressions of longitudinal polarization vectors have been used to determine the scattering cross-sections.
Generally, the idea of vector boson scattering has been used for a better understanding of EWSB.
A generic expression of the amplitude of the vector boson scattering has been given for these models.
From this analysis, it is revealed that away from resonance the cross-sections are not significantly different from that of the SM. This is quite expected because only those parameter spaces have been chosen which satisfy all the existing constraints.
One can differentiate these three models from the standard model and between one another, looking for the resonance peaks in different modes of vector boson scattering. In future, if we observe any signature of these new scalars in the future collider experiments, then this study will help in revealing the characteristics of the extended scalar sector.

 
If the standard model is valid up to the Planck scale, the present measurements on the masses of the top quark and Higgs indicate the presence of a deeper minimum of the scalar potential at a very high energy scale, threatening the stability of the present electroweak vacuum. State of the art NNLO calculations performed to evaluate the probability that the present EW vacuum will tunnel into the deeper vacuum lying close to $\mpl$ suggest that the present EW vacuum is metastable at $\sim$3$\sigma$. As a part of this thesis, this has been reproduced. The lack of stability might be the artifact of the incompleteness of the SM.

It is important to look into the problem of EW stability in a scenario which addresses the issue of DM as well. In this case, at a time an extended scalar sector has been taken which provides a viable dark matter candidate. In the presence of these new scalar sectors, the detailed study of the Higgs potential has been discussed.
Assuming these models valid up to the $\mpl$ scale and allowing the metastability of the electroweak vacuum, new viable parameter spaces have been found.
As new extra scalar sector introduces a few new parameters and fields, the study of the parameter space is quite involved when one considers radiatively improved scalar potentials containing SM NNLO corrections and two-loop new sector contributions.
Inclusion of these NNLO corrections is mandatory to reproduce the correct confidence level at which EW vacuum is metastable in the SM.
In these models, the formation of the extra minimum near the $\mpl$ scale have been described. The detailed calculation of transition probability from the EW minimum to the new minimum at the Planck scale has also been shown.
In the presence of new scalar sectors, the conditions for absolute stability of the EW vacuum have been reviewed in this work. If one allows the metastable EW vacuum then new metastability conditions arise which have also been shown for these extended scalar sectors of the SM.

As extra scalar sectors can provide a viable dark matter candidate which may fulfill the relic abundance of the dark matter in the Universe, in this context, it is instructive to explore whether these extra scalars can also extend the lifetime of the Universe. This study will help in estimating the mean lifetime of the EW vacuum, especially if it still remains in the metastable state in models with extended scalar sectors.


==> ssa/FirstPage.tex <==

\graphicspath{{FirstPage/}}
%\pagestyle{empty}
\pagestyle{plain}
 \pagenumbering{roman}\setcounter{page}{1}
\addcontentsline{toc}{section}{Title}


\begin{center}
\vspace*{-2 cm}
{\Large \textbf{Unitarity Bound on Extended Higgs  Sector with Higher Dimensional Operator}}\\


\vfill
{\large\textbf{M.Sc. Thesis}}\\
\vspace*{0cm}

\vfill\vspace*{0cm}
{\Large\textbf{by}}\\
\vspace*{0.5cm}
{\Large\textbf{DEEPAK}}\\
\vspace*{1cm}


\includegraphics[width=5cm,clip]{./Plots/IITimage}\\
\vspace*{2cm}

{\large\textbf{DISCIPLINE OF PHYSICS \\
    INDIAN INSTITUTE OF TECHNOLOGY INDORE \\
 JUNE, 2019}}\\
 
\vspace*{1cm}


\end{center}


\begin{center}
\newpage
\null
\newpage
\end{center}



\begingroup
\let\clearpage\relax
\let\cleardoublepage\relax
\let\cleardoublepage\relax




\begin{center}
\vspace*{-2.0cm}
{\Large \textbf{Unitarity Bound on Extended Higgs  Sector with Higher Dimensional Operator}}\\
\vspace*{0.3cm}
\vfill
{\large\textbf{A THESIS}}\\
\vspace*{0.3cm}

\vfill
{\large\it{Submitted in partial fulfillment of the \\requirements for the award of the degree}}\\
\vspace*{0.2cm}
{\large\textbf{$of$}}\\
\vspace*{0.5cm}

{\large\textbf{Master of Science}}\\
\vspace*{0.5cm}

\vfill\vspace*{0cm}
{\Large\textbf{by}}\\
\vspace*{0.7cm}
{\Large\textbf{DEEPAK}}\\
\vspace*{2cm}


\includegraphics[width=5cm,clip]{./Plots/IITimage}\\
\vspace*{2cm}

{\large\textbf{DISCIPLINE OF PHYSICS \\
    INDIAN INSTITUTE OF TECHNOLOGY INDORE \\
 JUNE, 2019}}\\
 
\vspace*{0.5cm}

\end{center}
\endgroup           

\vfill

\begin{center}
\newpage
\null

\end{center}
\begin{center}
\begin{figure}
		\includegraphics[width=18.7cm]{candia.jpg}
	\end{figure}
\end{center}
 \vspace*{-3.5cm}
  \thispagestyle{empty}
\begin{figure}[htbp]
\includegraphics[height=2.5cm,width=2.7cm]{./Plots/IITimage}
\end{figure}
\vspace{-2.5cm}
\begin{center} 
\hspace{2.7cm}{\Large\textbf{Indian Institute of Technology Indore}} 
\end{center}

\vspace{0.5cm}

%\noindent\parbox{\linewith}


%\vspace{-40pt}%if needed
\begin{center}
{\Large\textbf{CANDIDATE’S DECLARATION}}\\
%\pagestyle{plain}\addcontentsline{toc}{section}{CANDIDATE’S DECLARATION}
\phantomsection
\pagestyle{plain}\addcontentsline{toc}{section}{CANDIDATE’S DECLARATION}
\printindex
\end{center}
\vspace{2pt}
I hereby certify that the work which is being presented in the thesis entitled \textbf{Unitarity Bound on Extended Higgs  Sector with Higher Dimensional Operator} in the partial fulfillment of the requirements for the award of the degree of \textbf{MASTER OF SCIENCE} and submitted in the \textbf{DISCIPLINE OF PHYSICS, Indian Institute of Technology Indore,} is an authentic record of my own work carried out during the time period from July 2018 to June 2019 under the supervision of  Professor Subhendu Rakshit, IIT Indore.
\\The matter presented in this thesis has not been submitted by me for the award for any other degree of
this or any other institute.
	\vskip .2cm
\hspace*{8.3cm} {Signature of the student with date}
\hspace*{10.2cm} {\bf (DEEPAK)}\\
\noindent\hdashrule[0.5ex]{15.8cm}{0.8pt}{1mm}
This is to certify that the above statement made by the candidate is correct to the best of my knowledge.
\vspace{0.2cm}

\hspace*{7.3cm} {Signature of Thesis Supervisor with date}
\hspace*{8.3cm} {\bf (Prof. Subhendu Rakshit)}\\
\noindent\hdashrule[0.5ex]{15.8cm}{0.8pt}{1mm}
{\bf DEEPAK} has successfully given  his M.Sc. Oral  Examination held on {\bf 20 June, 2019}.
\vskip .1cm
\noindent
\mbox{{\bf Prof. Subhendu Rakshit}}  \hspace{4.9cm}\mbox{{ \bf Convener, DPGC}}\\
\mbox{Date:}  \hspace{9.1cm}\mbox{Date:}\\
\\
\mbox{{\bf Dr. Ankhi Roy}}      \hspace{7.0cm}\mbox{{\bf Dr. Bhargav Vaidya}}\\
\mbox{Date:}  \hspace*{9.1cm}\mbox{Date:}\\
\noindent\hdashrule[0.5ex]{15.8cm}{0.8pt}{1mm}
   


\clearpage
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\setstretch{1.3} % Reset the line-spacing to 1.3 for body text (if it has changed)

\newpage
\newpage
\null
\newpage

\vspace*{5cm}
{\Huge\textbf{ \hspace{4cm} Dedicated}}\\
        
      {\Huge\textbf{  \hspace{5.8cm} to}}\\
 
  {\Huge\textbf{ \hspace{3.8cm} My Family}}
\null
\newpage
\newpage
\null
\newpage
\begin{center}
{\Huge\textbf{Acknowledgements}}\\
%\pagestyle{plain}\addcontentsline{toc}{section}{Acknowledgements}

\phantomsection
\addcontentsline{toc}{section}{Acknowledgements}
\printindex


\end{center}
\vspace{28pt}
First and foremost, I gratefully acknowledge the continual guidance and support of my adviser, Prof. Subhendu Rakshit. His dedication to research and pursuit of
physics has been an invaluable source of inspiration and encouragement to me. His guidance helped me in all the time of research and writing of this thesis. 
\\I would like to thank my PSPC committee members, Dr. Ankhi Roy and Dr. Bhargav Vaidya for serving as my committee members even at hardship.
\\
It was not possible for me to achieve my M.Sc degree from an institute like IIT,
without the support of my family. I am very much thankful to my parents and
sisters for their constant support in my life.
\\
I would also like to thank all the research scholars working in Theoretical High
Energy Physics Lab for their co-operation and help during my M.Sc. research project.
\\
Special thanks to  Mr. Siddhartha Karmakar for valuable
guidance and support in thesis work.
\\
%Last but not least; I thank my friends Hridey Chetri, Rahul Kumar, Ravi Suman, Naveen Mendola, Debasish Sahoo, Manoj Kumar, Megha and Akansha Thakur for their help and motivation without which this would not have been possible.
%Finally, I would like to thank my friends  especially my best friend, Akansha Thakur
%for her continuous support and the cheerful Sunday coffee and pasta we shared.


% A big thank you is due to all my classmatesfor supporting me.




\newpage
\null
\newpage

\begin{center}
{\Huge\textbf{Abstract}}\\
%\pagestyle{plain}\addcontentsline{toc}{section}{Abstract}
\phantomsection
\addcontentsline{toc}{section}{Abstract}
\printindex
\end{center}
\vspace{28pt}

%\chapter*{Abstract \label{sec:abstract}}
%\pagestyle{plain}\addcontentsline{toc}{section}{Abstract}

We study the perturbative unitarity bound given by higher dimensional bosonic operators up to dim-6 for the two-Higgs-doublet model (2HDM). They lead to new physics beyond the Standard Model.  We point out that such operators can lead to a larger cross-section in the vector boson fusion channels for the scalars, compared to the tree-level 2HDM.
We have obtained limits on a few bosonic operators up to dim-6 for 2HDM, by ensuring unitarity of the  S-matrix.











